A Normalizing Intuitionistic Set Theory with Inaccessible Sets

We propose a set theory strong enough to interpret powerful type theories underlying proof assistants such as LEGO and also possibly Coq, which at the same time enables program extraction from its constructive proofs. For this purpose, we axiomatize an impredicative constructive version of Zermelo-Fraenkel set theory IZF with Replacement and $\omega$-many inaccessibles, which we call \izfio. Our axiomatization utilizes set terms, an inductive definition of inaccessible sets and the mutually recursive nature of equality and membership relations. It allows us to define a weakly-normalizing typed lambda calculus corresponding to proofs in \izfio according to the Curry-Howard isomorphism principle. We use realizability to prove the normalization theorem, which provides a basis for program extraction capability.

==> aczel.tex <==
  A standard set-theoretic function encoding works as follows. A function $f : A \to B$ is encoded
as a set of pairs $(a, b)$ such that $a \in A$, $b \in B$ and for all $a \in A$, there is exactly
one $b \in B$ such that $(a, b) \in f$. The application operation, $App(f, a)$ is then defined
as the unique $b$ such that $(a, b) \in f$. This encoding has a property that for all sets $A$, 
$\emptyset \in \emptyset \to A$.
  One disadvantage of this encoding is that in intuitionistic set theories, $App$ doesn't define
an operation. It is not the case that $\forall f, a \exists !b.\ App(f, a) = b$ ---
since App simply is not defined on sets which are not functions. Clasically, we can just
set it to $0$ on a set which is not a function, but intuitionistically we cannot decide if a set
is a function or not. 
  Aczel's encoding modifies the standard idea a little bit. Instead of storing a pair $(a, f(a))$ in a 
set encoding a function $f$, a pair $(a, b)$ is stored for every $b \in f(a)$. Formally, 
let's first define the application operation:
\[
App(f, a) \equiv \{ b\ |\ (a, b) \in f \} = \bigcup_{(a, b) \in f}\ \{ b \}
\]

Note that this operation is defined for all sets $f, a$. 

Then $A \to B$ is defined as the set of all $f$ such that:
\begin{itemize}
\item $f$ is a set of ordered pairs.
\item If $(a, b) \in f$, then $a \in A$.
\item For all $a \in A$, $App(f, a) \in B$.
\end{itemize}

The notion of dependent function product  $\Pi_{x \in A} B(x)$ is defined similarly
in an obvious way.

The first property of this encoding to notice is that not only for all $A$, $\emptyset \in 
\emptyset \to A$, but also for all $A$, $\emptyset \in A \to 1$. Indeed, let $a \in A$. 
Then $App(\emptyset, a)$ is the empty set and hence an element of $1$.

The more interesting property, essential to the correctness of Aczel's encoding of 
Prop as $P(1)$ in IZF is as follows:

\begin{lemma}
If for all $x \in A$, $B(x) \subseteq 1$, then $\Pi_{x \in A} B(x) \subseteq 1$. 
\end{lemma}

\begin{proof}
Take any $f \in \Pi_{x \in A} B(x)$. Then for all $a \in A$, $App(f, a) \in
B(a)$.
Since $B(a) \subseteq 1$, then for all $a \in A$, $App(f, a) \in 1$. So for all $a \in A$, 
$App(f, a) = 0$. Therefore, by the definition of $App$, for all $a \in A$, for all $b$, 
$(a, b) \notin f$. This entails that $f = \emptyset$ --- take any $c$ in $f$. Then $c$ is a pair
$(d, e)$, and $d \in A$, but we have just shown that it's not the case. So $f \in 1$, so $\Pi_{x \in A}
B(x) \subseteq 1$.  
\end{proof}

Once we have this property, we can validate the following proof rule for Prop:

\[
\infer{\forall x : A.\ \phi(x) : Prop}{x : A \proves \phi(x) : Prop}
\]

That is, Prop is closed under universal quantification over arbitrary domain. 
The similar thing for existential quantification can also be done, see below.

Moreover, this actually defines something close to the classical definition of truth for the universal quantifier,
as the following two lemmas show:

\begin{lemma}
If for all $x \in A$, $B(x) = 1$, then $\Pi_{x \in A} B(x) = 1$.
\end{lemma}
\begin{proof}
We already know that $\Pi_{x \in A} B(x) \subseteq 1$. All we need to show,
then, is that $\emptyset \in \Pi_{x \in A} B(x)$. But this is obvious, as for all
$a \in A$, $App(\emptyset, a) = \emptyset \in 1 = B(a)$. 
\end{proof}
 
\begin{lemma}
If there is $a \in A$ such that $B(a) = 0$, then $\Pi_{x \in A} B(x) = 0$.
\end{lemma}
\begin{proof}
If $f \in \Pi_{x \in A} B(x)$, then necessarily $App(f, a) \in B(a)$, so $App(f, a) \in \emptyset$,
but this is not the case. 
\end{proof}

The very interesting property of this encoding is that even though the product $\Pi_{x \in A} B(x)$, 
collapses set-theoretically to a subset of $1$, as we have just seen, the constructive
content is not lost, that is the following property still holds every time: If $f \in 
\Pi_{x \in A} B(x)$, then for all $a \in A$, there is (exactly one) $b \in B(a)$ such that
$App(f, a) = b$. Thus, using the IZF extraction we can still extract a function.
This is perhaps not so surprising in case of the universal quantification and Prop,
since proving that $f \in \Pi_{x \in A} B(x)$ amounts to proving that for all $a \in A$, $B(a) = 1$,
so the extracted function will follow from this fact and will not contain any interesting content.
However, things get interesting when we try to implement a dependent product in a similar way.
The standard set-theoretic interpretation of $\Sigma_{X \in A} B(x)$ is a set of a pairs $(a, b)$ such
that $a \in A$ and $b \in B(a)$. Let's, however, consider $\bigcup_{x \in A} B(x)$. We have the following
three properties, corresponding to ones for the Aczel's encoding of a dependent function product:

\begin{lemma}
If for all $a \in A$, $B(a) \subseteq 1$, then $\bigcup_{x \in A} B(x) \subseteq 1$.
\end{lemma} 
\begin{proof}
Suppose $c \in \bigcup_{x \in A} B(x)$. Then there is $a \in A$ such that $c \in B(a)$. 
So $c \in 1$.
\end{proof}

\begin{lemma}
If there is $a \in A$ such that $B(a) = 1$, then $\bigcup_{x \in A} B(x) = 1$. 
\end{lemma}
\begin{proof}
It suffices to show that $0 \in \bigcup_{x \in A} B(x)$, but $0 \in B(a)$ which 
shows the claim.
\end{proof}

\begin{lemma}
If for all $a \in A$ $B(a) = 0$, then $\bigcup_{x \in A} B(x) = 0$.
\end{lemma}
\begin{proof}
Suppose $c \in \bigcup_{x \in A} B(x)$. Then there is $a$ such that $c \in B(a)$.
But this is not the case.
\end{proof}

So suppose we have proof rules of the form:

\[
\infer{[a, M] : \exists x : A.\ \phi(x)}{ a : A & M : \phi(a)} \qquad
\infer{\exists x : A.\ \phi(x) : Prop}{x : A \proves \phi(x) : Prop}
\]

Then the set-theoretic semantics will validate this rule. The
translation of the dependent pair $[a, M]$ to set theory must
necessarily forget about $a$. However, even though set-theoretically $a$
is forgotten, it is not lost, as one can still recover $a$ from the 
IZF proof of the corresponding statement $\SB{M} \in
\bigcup_{x \in A}\ \SB{\phi(x)}$ (using term existence property of IZF).


==> conclusion.tex <==
\section{Further work}\label{conclusion}

  We have proved normalization, and thus DP, NEP, SEP and TEP for an
extension of \izfr\ strong enough to interpret ECC and CIC. Could the same
method be used for even stronger extensions? It should be relatively
straightforward to adapt our framework to tackle the axiom: ``For all $x$
there is $y$ such that $y$ is the smallest inaccessible containing $x$''. We
do not know, however, if the same thing can be done about Mahlo sets,
for which DP and NEP have been proven in \cite{frsce2}. 

{\bf Acknowledgements} I would like to thank my advisor, Bob Constable, for
support and helpful comments and Richard Shore for helpful discussions. 


==> further.tex <==
\section{Further work}\label{further}

We conjecture that normalization of IZF makes it possible to 
prove normalization of other systems via set-theoretic semantics. 

\begin{conjecture}
Any lambda-calculus with types with reasonable set-theoretic semantics weakly normalizes.
\end{conjecture}
\begin{proof}
(Sketch) Apply set-theoretic semantics and show that reduction steps in the calculus correspond to reduction steps in 
$\li$.
\end{proof}

The calculi amenable to this treatment would include in particular G\"odel's System T, Girard's
System F, Luo's ECC and Calculus of Inductive Constructions. 



==> hol.tex <==
\section{HOL}

In this section we define higher-order logic along with set-theoretic
semantics.

The types of HOL are generated by the following abstract grammar:

\[
\tau ::= nat\ |\ bool\ |\ (\tau_1, {\ldots} , \tau_n) |\ \tau \to \tau
\]

The terms of HOL are generated by the following abstract grammar:

\[
t ::= x_\tau\ |\ c_\tau \ |\ t_{\tau \to \sigma}\ t'_{\tau}\ |\ \lambda x_\tau.\ t_\sigma
\]

There are several distinguished constants of HOL:
\[
=_\alpha : (\alpha, \alpha) \to bool \qquad \Rightarrow : bool \to bool \to bool
\qquad \forall_\alpha : (\alpha \to bool) \to bool \qquad \exists_\alpha : (\alpha \to
bool) \to bool
\]
\[
\cup : (bool, bool) \to bool \qquad \cap : (bool,
bool) \to bool \qquad \bot : bool 
\]

\subsection{Semantics}

First recall that $0 = \emptyset$, $1 = \{ 0 \}$, $2 = \{ 0, 1 \}$. 

\begin{definition}
The environment $\rho$ is a function from variables to sets. 
\end{definition}

We first define a meaning $\SB{\tau}_\rho$ of a type $\tau$ in an
environment $\rho$ by structural induction on $\tau$. $\SB{\tau}_\rho$ is
equal to case $\tau$ of:
\begin{itemize}
\item $nat$ --- $\nat$
\item $bool$ --- $P(1)$
\item $(\tau_1, {\ldots} , \tau_n)$ --- $(\SB{\tau_1}_\rho, {\ldots} ,
\SB{\tau_n}_\rho)$
\item $\tau_1 \to \tau_2$ --- $\SB{\tau_1}_\rho \to \SB{\tau_2}_\rho$
\end{itemize}

Note --- classicaly $P(1) = 2$ which is what you would expect for a meaning
of $bool$. 

Then we define a meaning of a term $t$ by structural induction on $t$. Case
$t$ of:

\begin{itemize}
\item $x_\tau$ --- $\rho(x)$
\item $c_\tau$ --- $\rho(c)$
\item $t\ t'$ --- $App(\SB{t}\ \SB{t'})$
\item $\lambda x_\tau.\ t$ --- $\{ (a, \SB{t}_{\rho[x:=a]})\ |\ a \in
\SB{\tau}_\rho$
\end{itemize}

Finally, we define a standard environment assigning sets to all constants,
$\rho(c)$ = case $c$ of:

\begin{itemize}
\item $=_\alpha$ --- $\lambda (x_1, x_2).\ \{ x \in 1\ | \ x_1 = x_2 \}$
\item $\Rightarrow$ --- $\lambda (b_1, b_2).\ \{ x \in 1\ | \ x \in b_1 \to x
\in b_2 \}$
\item $\cup$ --- $\lambda (b_1, b_2).\ b_1 \cup b_2$
\item $\cap$ --- $\lambda (b_1, b_2).\ b_1 \cap b_2$
\item $\bot$ --- $0$
\item $T$ --- $1$
\item $\forall_\alpha$ --- $\lambda f.\ \bigcap_{a \in \SB{\alpha}} f(a)$
\item $\exists_\alpha$ --- $\lambda f.\ \bigcup_{a \in \SB{\alpha}} f(a)$
\end{itemize}

This is a standard semantics in a lattice of $P(1)$, with pseudo-complement
defined in the clause for the implication, which might look weird, but classically
it's equivalent to the standard truth-table semantics.

\subsection{Proof rules}

Choose some{\ldots} 

\subsection{Soundness}

Prove soundness wrt. semantics. That is, if $\proves \phi$, then $\SB{\phi} = \SB{true}$.

\section{Logic layer}

We have presented in the previous section a nice, concise system of
higher-order logic. This logic is good enough to formalize as much
mathematics as we want to. It is convenient, though, to use on top of it
a logic closer to the mathematical practice, with actual syntax for
quantifiers, understanding it as abbreviations for the actual HOL terms. 
Moreover, this is the only way to actually get extraction. All of this is
made formal below.

\begin{definition}
The formulas of $L$ are generated by the following abstract grammar:
\[
\phi ::= \forall x : \tau.\ \phi\ | \exists x : \tau.\ \phi\ |\ \phi \land
\phi\ \mbox{And other logical connectives}
\]
\end{definition}

So the only difference is that we actually have quantifiers on a lexical
level, instead of having them as built-in definitions. 

Now we define a translation $F$ of formulas of $L$ into HOL in a
straighforward way --- $F$ is identity on the propositional fragment 
and $F(\forall x : \tau. \phi) = \forall_\tau (\lambda x : \tau.\ F(\phi))$.

The advantage of using $L$ becomes clear once we define extraction mechanism.
We define a derived logical rules, using HOL primitives, which in HOL
implementation are simply tactics. We get some resulting logic, (hopefully) complete
wrt. HOL and provability relation. 
















==> izfreal1.tex <==
\newcommand\vl{V^{\lambda}}
\newcommand\vla{\vl_\alpha}
\newcommand\vlb{\vl_\beta}

\section{Realizability}\label{izfreal}

We move to define realizability for IZF. It's sufficient to work in 
IZF with Collection instead of Replacement. For our purposes, though,
the exact choic of the universe doesn't matter, so the reader can assume
that the universe models ZF, if that's the world she prefers. 

\subsection{$\la$}

We use a type-free version of lambda calculus for realizability. We call
this calculus $\la$. The terms of $\la$ are generated by the following grammar:

\[
M  ::=  x\ |\ M\ N\ |\ \lambda x.\ M\ |\ inl(M)
\]
\[
inr(M)\ |\ fst(M)\ | \ snd(M)\ | <M, N>
\]
\[
case(M, x.N, x.O)\ |\ axRep(M)\ |\ axProp(M)\ |\ ind'(M)
\]	

In other words, $\la$ is what's left from $\li$ after erasure of 
all first-order information. This can be made precise by the definition of
the erasure map from terms of $\li$ to $\la$, defined as follows:

\[
\ov{x} = x \qquad \ov{M\ N} = \ov{M}\ \ov{N} \qquad \ov{\lambda a. M}=\ov{M}
\]
\[
\ov{\lambda x : \tau. M} = \lambda x.\ \ov{M} \qquad \ov{inl(M)} =
inl(\ov{M}) 
\]
\[
\ov{[t, M]} = \ov{M} \qquad
\ov{<M, N>} = <\ov{M}, \ov{N}> \qquad
\ov{fst(M)} = fst(\ov{M})
\]
\[
\ov{magic(M)} = magic(\ov{M}) \quad \ov{let [a, y]=M\ in\ N} = (\lambda y.\ \ov{N})\ \ov{M}
\]
\[
\ov{axRep(t, \ov{u}, M)} = axRep(\ov{M})
\]
\[
\ov{axProp(t, \ov{u}, M)} = axProp(\ov{M})
\]
\[
\ov{ind'_\phi(M, \ov{t}, u)} = ind'(\ov{M})
\qquad
\ov{ind_\phi(M, \ov{t}, u)} = ind(\ov{M})
\]

We call a $\li$  reduction \emph{atomic} if it's of the form $(\lambda
a.\ M)\ t \to M[a:=t]$ and a $\li$ value \emph{atomic} if it's of the
form $\lambda a.\ M$. 

The reduction rules and values in $\la$ are induced in an obvious way from $\li$ --- 
if $M \to M'$ is a nonatomic reduction in $\li$, then $\ov{M} \to \ov{M'}$,
if $M$ is a nonatomic value in $\li$, then $\ov{M}$ is a value in $\la$. 
In particular, $ind'(M) \to M\ (\lambda x.\ ind'(M))$ and $ind(M) \to M\ (\lambda x.\ ind'(M))$.

\ifthenelse{\boolean{long}}
{
\begin{lemma}
$\ov{M[x:=N]} = \ov{M}[x:=\ov{N}]$
\end{lemma}
\begin{proof}
Induction on $M$.
\end{proof}

\begin{lemma}
$\ov{M[a:=t]} = \ov{M}$. 
\end{lemma}
\begin{proof}
Induction on $M$.
\end{proof}
}
{}

\begin{lemma}\label{erasurenorm}
If $\ov{M}$ normalizes, so does $M$. 
\end{lemma}
\begin{proof}
Any infinite chain of reductions starting from $M$ must contain infinite
chain of nonatomic reductions, which map to reductions in $\ov{M}$ in a
natural way. 
\end{proof}

\ifthenelse{\boolean{long}}
{
This proof can be easily made constructive.
}{}

\subsection{Realizability}

We assume some encoding of
$\la$-terms in set theory, i.e. as natural numbers. The set consisting of encoded $\la$-terms is denoted by 
$\Lambda$.

\begin{definition}
A set $A$ is a $\lambda$-name iff $A$ is a set of pairs $(v, B)$ such that
$v \in \Lambda$, $v$ is a value and $B$ is a $\lambda$-name.
\end{definition}

In other words, $\lambda$-names are sets hereditarily labelled by
$\la$ values.

\begin{definition}
A class of $\lambda$-names is denoted by $V^\lambda$. 
\end{definition}

Formally, $V_\lambda$ is generated by the following transfinite inductive
definition on ordinals:
\[
V^\lambda_\alpha = \bigcup_{\beta \lt \alpha} P(\la_v \times V^\lambda_\beta), 
\]
where $\la_v$ denotes the set of values in $\la$. Then $V^\lambda = \bigcup_{\alpha \in ORD}V^\lambda_\alpha$.
We reserve letters $A, B, C$ for $\lambda$-names. 

The $\lambda$-rank of a $\lambda$-name $A$ is the smallest $\alpha$ such
that $A \in \vla$. This notion can be formalized in IZF, as shown by Powell. 

\begin{definition}
If $\forall x \in A.\ \exists B.\ \phi(x, B)$, then $COLL(\phi, A)$ denotes
the lambda-name such that $\forall x \in A \exists B \in COLL(\phi, A).\
\phi(x, B)$. 
\end{definition}
The set $COLL(\phi, A)$ exists by Collection: Suppose that for all $x \in A$ there is $B$ such that $\phi(x, B)$. Then, by
Collection, there is a set $C$ such that for all $x \in A$ there is $B \in
C$ such that $\phi(x, B)$. Let $D = \{ b \in C\ |\ \exists x \in A.\ \phi(x,
b) \}$. Then $D$ is a set of $\lambda$-names. Let $E = \{ \lambda-rank(B)\
|\ B \in D \}$. $E$ exists by Replacement. Then $\gamma = max(E)$ is an ordinal such
that if $B \in D$, then $\lambda-rank(B) \leq \gamma$, so $B \in \vl_\gamma$, 
so $D \in \vl_{\gamma + 1}$, so $D$ is a $\lambda$-name. Take $COLL(\phi, A)
\equiv D$. 

\begin{definition}
A (class-sized) first-order language $L$ arises by enriching the IZF signature 
with constants for all $\lambda$-names.
\end{definition}

From now on until the end of this section, variables $M, N$ range exclusively over $\la$-terms, letters $a, b, c$ vary over 
logic variables in the language, 
and letter $\rho$ varies over finite partial functions from logic variables to
$V^\lambda$. We call such functions environments.

The number of function symbols in a term and formula, denoted by $fun(t)$
and $fun(\phi)$ is defined in a standard way, counting in case of $S_\phi$
and $R_\phi$ terms function symbols in $\phi$ as well. For example, $fun(S_{a = \bigcup
\omega}(P(P(\omega)))) = 5$. 

\begin{definition}
Let $\phi$ be a formula of $L$. By metalevel mutual induction we define a realizability relation $M
\reals_\rho \phi$ in an environment $\rho$ and a meaning of a term
$\SB{t}_\rho$ in an environment $\rho$. The definition is as follows:
\begin{enumerate}
\item $\SB{a}_\rho = \rho(a)$
\item $\SB{A}_\rho = A$
\item $\SB{\emptyset}_\rho = \emptyset$.
\item \label{omegadef} $\SB{\omega}_\rho = \omega'$, where $\omega'$ is defined by the means
of inductive definition: $\omega'$ is the smallest set in $\vl_\omega$ such that:
\begin{itemize}
\item For all $A$, if $M \reals A = 0$ and $O \downarrow inl(M)$, then
$(natRep(O), A) \in \omega'$. 
\item If $(M, A) \in \omega'$, then for all $B \in \vl_{\omega}$, for all $N$, if $N \reals B = \bigcup \{
A, \{A, A \} \}  \}$, $O \downarrow inr(P)$ and $P \downarrow <M, N>$, then $(natRep(O), B) \in \omega'$.
\end{itemize}
\item \label{termdef} $\SB{t_A(\ov{u})}_\rho = \{ (axRep(N),B) \in \la_v
\times \vl_\gamma |\ N \reals_\rho \phi_A(B, \SB{\ov{u}}_\rho)\}$.
\item $M \reals_\rho t \in s \equiv M \downarrow v \land (v, \SB{t}_\rho) \in \SB{s}_\rho$
\item $M \reals_\rho \phi \land \psi \equiv M \downarrow <M_1, M_2> \land M_1
\reals_\rho \phi \land M_2 \reals_\rho \psi$
\item $M \reals_\rho \phi \lor \psi \equiv (M \downarrow inl(M_1) \land M_1
\reals_\rho \phi) \lor (M \downarrow inr(M_1) \land M_1 \reals_\rho \psi)$
\item $M \reals_\rho \phi \to \psi \equiv (M \downarrow \lambda x.\ M_1) \land
\forall N.\ (N \reals_\rho \phi) \to (M_1[x:=N] \reals_\rho \psi)$
\item $M \reals_\rho \forall a.\ \phi \equiv M \downarrow v \land \forall A \in
V^\lambda.\ v \reals_\rho \phi[a:=A]$
\item $M \reals_\rho \exists a.\ \phi \equiv M \downarrow v \land \exists A \in
V^\lambda.\ v \reals_\rho \phi[a:=A]$
\end{enumerate}
\end{definition}

The ordinal $\gamma$ in the case \ref{termdef} of the definition is defined
depending on the term $t_A(\ov{u})$. Let $\ov{\alpha} = \ov{rank(\SB{u}_\rho)}$. 
Case $t_A(\ov{u})$ of:
\begin{itemize}
\item $\{ u_1, u_2 \}$ --- $\gamma = max(\alpha_1, \alpha_2)$
\item $P(u)$ --- $\gamma = \alpha + 1$. 
\item $\bigcup u$ --- $\gamma = \alpha$.
\item $sep_{\phi}(u, \ov{u})$ --- $\gamma = \alpha_1 + 1$.
\item $repl_{\phi(x, y, \ov{f})}(u, \ov{u})$. This case is more complicated.
Let $C = \{ (N, (P, A)) \in \Lambda \times \SB{u}_\rho\ |\ \exists B.\ N
\downarrow \lambda x.\ O \land O[x:=P] \reals_\rho \phi(A, B, \ov{u}_\rho)
\}$. Then for all $c \in C$ there is $B$ and $(N, (P, A))$ such that $c =
(N, (P, A))$ and $N \downarrow \lambda x.\ O \land O[x:=P] \reals_\rho \phi(A, B, \ov{u}_\rho)$.
By Collection, there is an ordinal $\alpha$ such that for all $c \in C$
there is $B \in \vl_\alpha$ and $(N, (P, A))$ such that $c =
(N, (P, A))$ and $N \downarrow \lambda x.\ O \land O[x:=P] \reals_\rho
\phi(A, B, \ov{u}_\rho)$. Take $\gamma = \alpha + 1$.
\end{itemize}


The induction in this definition is on the mesaure function $m$, which takes a clause in the
definition and returns a quadruple of integers in the following way:
\begin{itemize}
\item $m(M \reals_\rho \phi)$ = (``number of constants $\omega$ in $\phi$'',
``$fun(\phi)$'', ``number of $=$ symbols in $\phi$'', ``structural complexity of $\phi$'')
\item $m(\SB{t}_\rho)$ = (``number of constants $\omega$ in $t$'', ``$fun(t)$'', 0, 0)
\end{itemize}
With lexicographical order in $\nat^4$, it's trivial to check that the measure
of the definiendum is always greater than the measure of the definiens ---
number of terms stays the same in clauses for realizability and formula
complexity goes down, in the clause for equality one quality symbol disappears, 
in the clause for $\omega$, $\omega$ disappears, and in the rest of clauses for terms,
one function symbol (the topmost one) disappears.

Since the definition is well-founded, (metalevel) inductive proofs on the
definition of realizability are justified.


\begin{lemma}\label{ineqrank}
If $A \in \vla$, then there is $\beta \lt \alpha$ such that
for all $t$, if $M \reals_\rho t \in A$, then $\SB{t}_\rho \in \vlb$. Also, if $M
\reals_\rho B = A$, then $B \in \vla$. 
\end{lemma}
\begin{proof}
Take $A \in \vla$. Then there is $\beta \lt \alpha$ such that $A \in P(\la_V \times
\vlb)$. Take any $B$. If $M \reals B \in A$, then $M \downarrow v$ and $(v,
B) \in A$, so $B \in \vlb$. 

For the second part, suppose $M \reals_\rho A = B$. Then $M \downarrow extRep(N)$ and 
$N \reals_\rho \forall c.\ c \in A \iffl c \in B$, so $\forall C.\ N \reals C \in A \iffl C \in B$, so $\forall
C.\ N \downarrow <N_1, N_2>$ and $N_1 \reals C \in A \to C \in B$ and $N_2
\reals C \in B \to C \in A$. Now take any elemend $(v, D) \in B$. Then $v
\reals D \in B$, so $N_2\ v \reals D \in A$, so $N_2\ v \downarrow v_1$ and
$(v_1, D) \in A$, so $(v_1, D) \in \la_v \times \vlb$. Therefore $B
\subseteq \la_v \times \vlb$, so $B \in P(la_v \times \vlb)$, so $B \in
\vla$. 
\end{proof}

\begin{lemma}
$(M, A) \in \SB{t_A(\ov{u})}_\rho$ iff $M = axRep(N)$ and $N \reals_\rho
\phi_A(A, \SB{\ov{u}}_\rho)$.
\end{lemma}

\begin{proof}
Left-to-right direction is immediate. For the right-to-left direction,
suppose $N \reals_\rho \phi_A(A, \SB{\ov{u}}_\rho)$ and $M = axRep(N)$. To
show that $(M, A) \in \SB{t_A(\ov{u})}_\rho$, we need to show that $A
\in \vl_{f_A(\ov{rank(\SB{\ov{u}})})}$.  The proof proceeds by case analysis
on $t_A(\ov{u})$. Let $\ov{\alpha} = \ov{rank(\SB{u}_\rho)}$. Case $t_A(\ov{u})$ of:

\begin{itemize}
\item $\{ u_1, u_2 \}$. Suppose that $N \reals_\rho A = \SB{u_1}_\rho \lor A
= \SB{u_2}_\rho \}$. Then either $(N \downarrow\ inl(N_1) \land N_1 \reals_\rho A =
\SB{u_1}_\rho)$ or $(N \downarrow\ inl(N_1) \land N_1 \reals_\rho A =
\SB{u_2}_\rho \}$. By Lemma \ref{ineqrank}, in the former case $A \in
\vl_{\alpha_1}$, in the latter $A \in \vl_{\alpha_2}$, so $A \in
\vl_{max(\alpha_1, \alpha_2)}$. 
\item $P(u)$. Suppose that $N \reals \forall c.\ c\ \in A \to c \in
\SB{u}_\rho$. Then $N \downarrow N_1 \land \forall C.\ N_1 \reals C \in A
\to C \in \SB{u}_\rho$, so $N \downarrow N_1 \land \forall C.\ N_1 \downarrow \lambda x.\ N_2 \land \forall M.\ (M \reals
C \in A) \Rightarrow N_2[x:=M] \reals C \in \SB{u}_\rho$.
Take any $(v, B) \in A$. Then $v \reals B \in A$. So $N_2[x:=v] \reals B \in \SB{u}_\rho$.
Thus any such $B$ is in $\vl_{\alpha}$, so $A \in \vl_{\alpha + 1}$.
\item $\bigcup u$. Suppose $N \reals \exists c.\ c \in \SB{u}_\rho \land A
\in c$. It's easy to see that $A \in \vla$. 
\item $sep_\phi(u, \ov{u})$.  Suppose $N \reals A \in \SB{u}_\rho \land {\ldots}$.
It follows that $A \in \vla$.
\item $repl_\phi(u, \ov{u})$. Suppose $N \reals (\forall x \in \SB{u}_\rho \exists! y.\ \phi(x,
y, \ov{\SB{u}_\rho})) \land \exists x \in \SB{u}_\rho.\ \phi(x, A, \ov{\SB{u}_\rho}) \}$. Then $N \downarrow
<N_1, N_2>$ and $N_1 \reals \forall x \in \SB{u}_\rho \exists! y.\ \phi(x, y, \ov{\SB{u}_\rho})$
and $N_2 \reals \exists x \in \SB{u}_\rho.\ \phi(x, A, \ov{\SB{u}_\rho})$. So for all $B$, $N_1 \downarrow
\lambda x.\ O$ and for all $P \reals B \in \SB{u}_\rho$, $O[x:=P] \reals \exists !y.\
\phi(B, y, \ov{\SB{u}_\rho})$. So for all $B$, $N_1 \downarrow
\lambda x.\ O$ and for all $P \reals B \in \SB{u}_\rho$, there is $C$ such that
$O[x:=P] \reals \phi(B, C, \ov{\SB{u}_\rho}) \land \forall d.\ \phi(B, d, \ov{\SB{u}_\rho}) \to
d = C$. So for all $(P,B) \in \SB{u}_\rho$, 
there is $C$ such that $N_1 \downarrow \lambda x.\ O$ and $O[x:=P]\ \reals
\phi(B, C, \ov{\SB{u}_\rho}) \land \forall d.\ \phi(B, d, \ov{\SB{u}_\rho})
\to d = C$. Thus $(N, (P, B)) \in E$, so any such $C$ is in $\vl_\gamma$. 
that {\ldots} 

Now there is $B$ such that $M_2 \reals B \in \SB{u}_\rho \land \phi(B, A, \ov{\SB{u}_\rho})$. So $M_2 \downarrow
<M_{21}, M_{22}>$ and $M_{21} \reals B \in \SB{u}_\rho$ and $M_{22} \reals \phi(B, A,
\ov{\SB{u}_\rho})$. Therefore, $N[x:=M_{21}] \reals \phi(B, C, \ov{\SB{u}_\rho}) \land \forall d.\ \phi(B, d, \ov{\SB{u}_\rho}) \to
d = C$. So $N[x:=M_{21}] \downarrow <O_1, O_2>$ and $O_1 \reals \phi(B, C,
\ov{\SB{u}_\rho})$ and $O_2 \reals \forall d.\ \phi(B, d, \ov{\SB{u}_\rho}) \to
d = C$. Therefore, $O_2 \downarrow \lambda x.\ P$ and $P[x:=M_{22}] \reals A
= C$. So by Lemma \ref{ineqrank}, any such $A$ is in $\vl_\gamma$, too, so
$\SB{repl_\phi(\SB{u}_\rho, \ov{\SB{u}_\rho})}_\rho \in \vl_{\gamma + 1}$.
\end{itemize}
\end{proof}

\begin{lemma}\label{realsubst1}
$\SB{t[a:=s]}_\rho = \SB{t}_{\rho[a:=\SB{s}_\rho]}$ and $M \reals_\rho \phi[a:=s]$ iff $M \reals_{\rho[a:=\SB{s}_\rho]} \phi$.
\end{lemma}
\begin{proof}
Induction on the definition of realizability. 
\ifthenelse{\boolean{long}}
{
Case $t$ of:
\begin{itemize}
\item $A$. Then both sides are equal to $A$. 
\item $a$. Then $\SB{t[a:=s]}_\rho = \SB{s}_\rho = \SB{a}_{\rho[a:=\SB{s}_\rho]}$
\item $b$. Then $\SB{t[a:=s]}_\rho = \rho(b) = \SB{b}_{\rho[a:=\SB{s}_\rho]}$
\item $t_A(\ov{u})$. Then $\SB{t[a:=s]}_\rho = \{ (axRep(N), A)\ |\ N \reals
\phi_A(A, \ov{u}[a:=s]) \}$. By IH, this is equal to $\{ (axRep(N), A)\ |\ N
\reals_{\rho[a:=\SB{s}_\rho]} \phi_A(A, \ov{u}) \} =
\SB{t}_{\rho[a:=\SB{s}_\rho]}$
\item $\omega$. The proof is trivial.
\end{itemize}
Case $\phi$ of:
\begin{itemize}
\item $t \in u$. Then $M \reals_\rho \phi[a:=s]$ iff $M \reals_\rho t[a:=s]
\in u[a:=s]$ iff $M \downarrow v$ and $(v, \SB{t[a:=s]}_\rho) \in
\SB{u[a:=s]})\rho$ iff (by IH) $(v, \SB{t}_{\rho[a:=\SB{s}_\rho])} \in
\SB{u}_{\rho[a:=\SB{s}_\rho]}$ iif $M \reals_{\rho[a:=\SB{s}_\rho])} t \in
u$ which is what we want.
\item The inductive steps are trivial. 
\end{itemize}
}{}
\end{proof}

\begin{lemma}\label{realsubst2}
$\SB{t[a:=s]}_\rho = \SB{t[a:=\SB{s}_\rho]}_\rho$ and $M \reals_\rho
\phi[a:=s]$ iff $M \reals_\rho \phi[a:=\SB{s}_\rho]$.
\end{lemma}
\begin{proof}
Induction on the definition of realizability. 
\ifthenelse{\boolean{long}}
{
Case $t$ of:
\begin{itemize}
\item $A$. Then both sides are equal to $A$. 
\item $a$. Then $\SB{t[a:=s]}_\rho = \SB{s}_\rho = \SB{\SB{s}_\rho} =
\SB{t[a:=\SB{s}_\rho]}$. 
\item $b$. Then both sides are euqal to $\SB{b}_\rho$. 
\item $t_A(\ov{u})$. Then $\SB{t[a:=s]}_\rho = \{ (axRep(N), A)\ |\ N \reals
\phi_A(A, \ov{u}[a:=s]) \}$. By IH, this is equal to $\{ (axRep(N), A)\ |\ N
\reals_\rho \phi_A(A, \ov{u}[a:=\SB{s}_\rho]) \} =
\SB{t_a(\ov{u}}[a:=\SB{s}_\rho]$.
\end{itemize}
Case $\phi$ of:
\begin{itemize}
\item $t \in u$. Then $M \reals_\rho \phi[a:=s]$ iff $M \downarrow v$ and
$(v, \SB{t[a:=s]}_\rho) \in \SB{u[a:=s]}_\rho$ iff (by IH)
$(v, \SB{t[a:=\SB{s}_\rho]}_\rho) \in \SB{u[a:=\SB{s}_\rho]}_\rho$ iff
$M \reals_\rho t[a:=\SB{s}_\rho] \in \SB{u[a:=\SB{s}_\rho]}$, which is what
we want.
\item The inductive cases are trivial. 
\end{itemize}
}{}
\end{proof}
\begin{lemma}
If $(M \reals_\rho \phi)$ then $M \downarrow$.
\end{lemma}
\ifthenelse{\boolean{long}}
{
\begin{proof}
Immediate. 
\end{proof}
}
{}

\ignore
{
\begin{lemma}
$IZF \proves M \downarrow$ iff $M \downarrow$. 
\end{lemma}
\begin{proof}
One direction follows from $V \models IZF$, the other from the fact that $M
\downarrow$ is a $\Sigma_1$-sentence and $IZF$ formalizes arithmetic. 
\end{proof}
}
\begin{lemma}\label{realredclosed}
If $M \to^* M'$ then $M'\reals_\rho \phi$ iff $M \reals_\rho \phi$.
\end{lemma}
\begin{proof}
Whether a term $N$ realizes a formula or not depends only on the behavior
of the values, which don't change with reduction/expansion, since the
reduction is deterministic.
\end{proof}
\begin{lemma}\label{realimpl}
If $M \reals_\rho \phi \to \psi$ and $N \reals_\rho \phi$, then $M\ N \reals
\psi$. 
\end{lemma}
\begin{proof}
Suppose $M \reals_\rho \phi \to \psi$. Then $M \downarrow (\lambda x. O)$
and for all $P \reals \phi$, $O[x:=P] \reals \psi$. Now, $M\ N \to^*
(\lambda x. O) N \to O[x:=N]$. Lemma \ref{realredclosed} gives us the claim. 
\end{proof}

\begin{lemma}\label{realomega}
$(natRep(O), B) \in \omega'$ iff $O \reals B = 0 \lor \exists y.\ y \in
\omega'.\ B = S(y)$.
\end{lemma}
\begin{proof}
For left-to-right direction we proceed by induction on the definition of $\omega'$:
\begin{itemize}
\item The base case. Then $O \downarrow inl(M)$ and $M \reals B = 0$. The claim is
trivial. 
\item Inductive step. Then $O \downarrow inr(<M, N>)$, $(M, A) \in \omega'$, $N \reals
B = \bigcup \{ A, \{ A, A \} \}$. Therefore there is $C$ (namely $A$) such
that $M \reals C \in \omega'$ and $N \reals B = \bigcup \{ C, \{ C, C \} \}$. 
Thus $inr(<M, N>) \reals B = 0 \lor \exists y.\ y \in
\omega'.\ B = S(y)$, so also $O \reals B = 0 \lor \exists y.\ y \in
\omega'.\ B = S(y)$. 
\end{itemize}
For right-to-left direction, suppose $O \reals B = 0 \lor \exists y. y \in
\omega' \land O = \bigcup \{ y, \{ y, y \} \}$. Then either $O \downarrow
inl(M)$ or $O \downarrow inr(P)$. In the former case, $M \reals B = 0$, so
indeed $(natRep(O), B) \in \omega'$. In the latter, $P \reals \exists y.\ y \in
\omega' \land B = \bigcup \{ y, \{ y, y \} \}$. So there is $A$ such that $P
\reals A \in \omega' \land B = \bigcup \{ A, \{ A, A \} \}$. So $P
\downarrow <M, N>$ and $(M, A) \in \omega'$ and $N \reals B = \bigcup \{ A,
\{ A, A \} \}$, which is exactly what the inductive step of the definition
of $\omega'$ consists of. This ends the proof. 
\end{proof}

\ifthenelse{\boolean{long}}
{
\input{explainreal}
}{}


==> lei.tex <==
\section{Extensional IZF}\label{lei}

We will show that we can extend our results to full IZF. We work in \iizf.

\begin{lemma}
Equality is an equivalence relation.
\end{lemma}

\ignore
{

Beeson's belief that Leibniz axiom is never used in mathematical practice is
deeply mistaken, as we have found out formalizing small parts of set theory.
Leibniz axiom is used all over the place. 
}

\begin{definition}
A set $C$ is \emph{L-stable}, if $A \in C$ and $A = B$ implies $B \in
C$. 
\end{definition}

\begin{definition}
A set $C$ is \emph{transitively L-stable} if it is L-stable and every
element of $C$ is L-stable. 
\end{definition}

This definition is formalized in a standard way, using transitive closure, available
in \iizf, as shown i.e. in \cite{ar}. We write $TLS(A)$ to express that $A$ is
transitively L-stable and denote the class of transitively L-stable sets
by $T$. The statement $V=T$ means that $\forall A.\ TLS(A)$. Class $T$ in \iizf
plays a similar role to the class of well-founded sets in ZF without
Foundation. 

\begin{lemma}
IZF $\p V=T$. 
\end{lemma}
\begin{proof}
By $\in$-induction. 
\end{proof}

The restriction of a formula $\phi$ to $T$, denoted by $\phi^T$, is defined
as usual, taking into account the following translation of terms:
\[
a^T \equiv a \quad \{ t, u \}^T \equiv \{ t^T, u^T \} \qquad \omega^T \equiv \omega \qquad
(\bigcup t)^T \equiv \bigcup t^T \qquad
\]
\[
(P(t))^T \equiv P(t^T) \cap T \qquad (S_{\phi(a, \ov{f})}(u, \ov{u}))^T \equiv S_{\phi^T(a, \ov{f})}(u^T,
\ov{u^T}) 
\]
\[
(R_{\phi(a, b, \ov{f})}(t, \ov{u}))^T \equiv R_{b \in T \land \phi^T(a, b,
\ov{f})}(t^T, \ov{u^T})
\]
The notation $T \models \phi$ means that $\phi^T$ holds.
\begin{lemma}
$T$ is transitive. 
\end{lemma}
\ifthenelse{\boolean{long}}
{
\begin{proof}
Take any $A$ in $T$ and suppose $a \in A$. Then also $a \in T$, by the
definition of $T$. 
\end{proof}
}{}

\begin{lemma}\label{t1}
If $A=C$ and $A \in T$, then $C \in T$. 
\end{lemma}
\ifthenelse{\boolean{long}}
{
\begin{proof}
Suppose $a \in C$ and $a = b$. Since $A=C$, $a \in A$. Since $A$ is
L-stable, $b \in A$, so also $b \in C$. Thus $C$ is L-stable. 

If $a \in C$, then $a \in A$. Since $A \in T$ and $T$ is transitive then $a
\in T$. Thus $C$ is transitively L-stable. 
\end{proof}
}{}

\ifthenelse{\boolean{long}}
{
\begin{proof}
This is not obvious, since there is no $L$ axiom in the logic. However,
equality is defined by $\Delta_0$-formula and the claim follows by transitivity of $T$.
\end{proof}

We refrain from making claims regarding absoluteness of terms, as the
concept is a bit fishy in the universe without the Leibniz axiom.
}
{
}

\begin{lemma}\label{tlstable}
$T \models$ ``every set is L-stable''.
\end{lemma}

\begin{lemma}
Equality is absolute for $T$. 
\end{lemma}

The following three lemmas are proved together by mutual induction on the
definition of terms and formulas. 


\begin{lemma}\label{trieq}
For any term $t(a, \ov{f})$, $T \models \forall a, b, \ov{f}.\ a = b \to
t(a, \ov{f}) = t(b, \ov{f})$.
\end{lemma}
\ifthenelse{\boolean{long}}
{
\begin{proof}

Case $t(a, \ov{f})$ of:
\begin{itemize}

\item $a$, $f_i$ or $\omega$. The claim is trivial.

\item $\{ t_1(a, \ov{f}), t_2(a, \ov{f}) \}$. By IH, $t_1^T(a, \ov{f}) =
t_1^T(b, \ov{f})$ and $t_2^T(a, \ov{f}) = t_2^T(b, \ov{f})$. 
Take any $A \in \{ t_1^T(a, \ov{f}), t_2^T(a, \ov{f}) \}$. Then
either $A = t_1^T(a, \ov{f})$ or $A = t_2^T(a, \ov{f})$, so either
$A = t_1^T(b, \ov{f})$ or $A = t_2^T(b, \ov{f})$, in both cases $A \in \{
t_1^T(b, \ov{f}) , t_2^T(b, \ov{f}) \}$. The other direction is symmetric.
\item $\bigcup t(a, \ov{f})$. By IH, $t^T(a, \ov{f}) = t^T(b, \ov{f})$. Take any
$A \in \bigcup t^T(a, \ov{f})$. Then there is $B \in t^T(a, \ov{f})$ such that
$A \in B$. So also $B \in t^T(b, \ov{f})$, so $A \in \bigcup t^T(b,
\ov{f})$. The other direction is symmetric. 
\item $S_{\phi(a, \ov{f})}(t(a, \ov{f}), \ov{t(a, \ov{f})})$. Suppose $A \in
S^T_{\phi(a, \ov{f})}(t^T(a, \ov{f}), \ov{t^T(a, \ov{f})})$. Then $A \in t^T(a,
\ov{f}) \land \phi^T(A, \ov{t^T(a, \ov{f})})$. By IH, $t^T(a, \ov{f}) =
t^T(b, \ov{f})$, so $A \in t^T(b, \ov{f})$. Also by IH, $\ov{t^T(a, \ov{f})}
= \ov{t^T(b, \ov{f})}$. By Lemma \ref{tril}, $\phi^T(A, \ov{t^T(b,
\ov{f})})$. Thus $A \in S^T_{\phi(a, \ov{f})}(t^T(b, \ov{f}), \ov{t^T(b,
\ov{f})})$.
On the other hand, if $A \in S^T_{\phi(a, \ov{f})}(t^T(b, \ov{f}), \ov{t^T(b,
\ov{f})})$, then $A \in t^T(b, \ov{f})$, so also $A \in t^T(a, \ov{F})$, and
$\phi^T(A, \ov{t^T(b, \ov{f})})$, so also $\phi^T(A, \ov{t^T(a, \ov{F})})$.
\item $R_{\phi(a, b, \ov{f})}$. Suppose $A \in R^T_{\phi(a, b,
\ov{f})}(t(a, \ov{f}), \ov{u(a, \ov{f})})$. This means that:

\begin{itemize}
\item $\forall x \in a \exists !y \in T.\ \phi^T(x, y, \ov{u^T(a, \ov{f})})$.
Take any $x \in A$. Then there is $y \in T$ such that $\phi^T(x, y,
\ov{u^T(a, \ov{f})})$ and $\forall z \in T.\ \phi^T(x, z, \ov{u^T(a,
\ov{f})}) \to z = y$. Take any $x' \in A$. Let $y' = y$. 
By IH, $\ov{u^T(a, \ov{f})} = \ov{u^T(b, \ov{f})}$, so by 
By Lemma \ref{tril}, $\phi^T(x, y, \ov{u^T(b, \ov{f})})$.
Take any $z \in T$ and assume $\phi^T(x, z, \ov{u^T(b, \ov{f})})$. By Lemma
\ref{tril}, $\phi^T(x, z, \ov{u^T(a, \ov{f})})$, so $z = y = y'$. 
\item $\exists x \in a.\ \phi^T(x, A, \ov{u^T(a, \ov{f})})$. Since by Lemma
\ref{tril}, $\phi^T(x, A, \phi^T(x, A, \ov{u^T(a, \ov{f})}))$ implies
$\phi^T(x, A, \ov{u^T(b, \ov{f})})$, there is $x \in a$ such that $\phi^T(x,
A, \ov{u^T(b, \ov{f})})$.
\end{itemize}
So, altogether, $A \in R_{\phi(a, b, \ov{f})}(t^T(b, \ov{f}),
\ov{u^T(b, \ov{f})})$. 

The other direction, as always, is symmetric.
\end{itemize}
\end{proof}
}{}

\begin{lemma}\label{tritint}
For any term $t(a, \ov{f})$, $\forall a, \ov{f} \in T.\ \ t^T(a, \ov{f}) \in T$.
\end{lemma}
\ifthenelse{\boolean{long}}
{
\begin{proof}
As this time luckily the exact form of subterms has no relevance, to increase
readability we will denote them by capital letters. Case $t(a, \ov{f})$ of:
\begin{itemize}
\item $a$ or $f_i$. The claim is trivial. 
\item $\{ A, B \}$. By IH, $A, B \in T$.
Take $C, D$, $C = D$, $C \in \{ A, B \}$. 
Then $C = A$ or $C = B$, so $D = A$ or $D = B$, so $D \in \{ A, B \}$. Thus
$\{ A, B \} \in T$.
\item $\bigcup A$. By IH, $A \in T$. Take $C \in \bigcup A$, then there is
$B \in A$ such that $C \in B \in A$. By transitivity of $T$, $B \in T$, so
$C \in T$. Suppose $C = D$. Since $B \in T$, then $D \in T$, so $D \in
\bigcup A$. 
\item $S_{\phi(a, \ov{f})}(A, \ov{F})$. By IH $A, \ov{F} \in T$. Suppose $a \in \{ x
\in A\ |\ \phi^T(x, \ov{F}) \}$. Then $a \in A$, so $a \in T$. Suppose $a = b$. We have $a \in A$
and $\phi^T(a, \ov{F})$. By $A \in T$, $b \in A$. By Lemma \ref{tril},
$\phi^T(b, \ov{F})$. So $b \in \{ x \in A\ |\ \phi^T(x, \ov{F}) \}$.
\item $R_{\phi(a, b, \ov{f})}(A, \ov{F})$. By IH $A, \ov{F} \in T$. Suppose
$b \in R_{b \in T \land \phi^T(a, b, \ov{f})}(A, \ov{F})$. Then:
\begin{enumerate}
\item For all $x \in A$ there is exactly one $y \in T$ such that $\phi^T(x,
y, \ov{F})$.
\item There is $x \in A$ such that $b \in T$ and $\phi^T(x, b, \ov{F})$. 
\end{enumerate}
Therefore $b \in T$. Suppose $b = c$. Item 1 still holds. By Lemma \ref{t1},
$c \in T$. Lemma \ref{tril} gives us $\phi^T(x, c, \ov{F})$.
\end{itemize}
\end{proof}
}{}

\begin{lemma}\label{tril}
$T \models L_{\phi(a, \ov{f})}$.
\end{lemma}
\begin{proof}
\ifthenelse{\boolean{long}}
{Case $\phi$ of:}{The only interesting case is when $\phi$ is atomic.
Suppose }
\ifthenelse{\boolean{long}}
{
\begin{itemize}
\item}{} $t(A, \ov{F}) \in s(A, \ov{F})$ for some terms $t, s$. We need to show
that if $A, B \in T$, $A = B$ and $t^T(A, \ov{F}) \in s^T(A, \ov{F})$, then $t^T(B,
\ov{F}) \in s^T(B, \ov{F})$. By Lemma \ref{trieq}, $t^T(A, \ov{F}) =
t^T(B, \ov{F})$. By Lemma \ref{tritint}, $s^T(A, \ov{F}) \in T$, so by Lemma
\ref{tlstable} $t^T(B, \ov{F}) \in s^T(A, \ov{F})$. By Lemma \ref{trieq}, $s^T(A, \ov{F}) =
s^T(B, \ov{F})$, so $t^T(B, \ov{F}) \in s^T(B, \ov{F})$.
\ifthenelse{\boolean{long}}
{
\item $\bot$. Take any $a, b, \ov{c}$ and assume $a = b$ and $\bot$. Then
obviously $\bot$ holds as well.
\item $\phi_1(x, \ov{y}) \land \phi_2(x, \ov{y})$. Take any $a,
b, \ov{c}$, assume $a = b$ and $\phi_1(a, \ov{c})$ and
$\phi_2(a, \ov{c})$. By inductive hypothesis for $\phi_1$, we get
$\phi_1(b, \ov{c})$, by inductive hypothesis for $\phi_2$, we get
$\phi_2(b, \ov{c})$, so we get $\phi_1(b, \ov{c}) \land
\phi_2(b, \ov{c})$ which is what we need.
\item $\phi_1(x, \ov{y}) \lor \phi_2(x, \ov{y})$. Take any $a,
b, \ov{c}$, assume $a = b$ and $\phi_1(a, \ov{c}) \lor
\phi_2(a, \ov{c})$. If we have $\phi_1(a, \ov{c})$, then
by inductive hypothesis for $\phi_1$, we get 
$\phi_1(b, \ov{c})$, so also $\phi_1(b, \ov{c}) \lor
\phi_2(b, \ov{c})$. If we have $\phi_2(a, \ov{c})$, then by inductive hypothesis for $\phi_2$, we get
$\phi_2(b, \ov{c})$, so also $\phi_1(b, \ov{c}) \lor
\phi_2(b, \ov{c})$. In both cases we get $\phi_1(b, \ov{c}) \lor
\phi_2(b, \ov{c})$ which is what we need.
\item $\phi_1(x, \ov{y}) \to \phi_2(x, \ov{y})$. Take any $a,
b, \ov{c}$, assume $a = b$ and $\phi_1(a, \ov{c}) \to
\phi_2(a, \ov{c})$ and $\phi_1(b, \ov{c})$. By inductive
hypothesis for $\phi_1$ applied with $a, b$ exchanged, we get $\phi_1(a,
\ov{c})$. By the assumption, we have $\phi_2(a, \ov{c})$. By inductive
hypothesis for $\phi_2$ we get $\phi_2(b, \ov{c})$ which is what we need.
\item $\forall z.\ \phi_1(x, \ov{y}, z)$. Take any $a, b, \ov{c}$, assume $a
= b$ and $\forall z.\ \phi_1(a, \ov{c}, z)$ and take any $z$. We have to
show that $\phi_1(b, \ov{c}, z)$ holds. By inductive hypothesis for
$\phi_1$, with $z$ merged into $\ov{y}$, we get the claim easily.
\item $\exists z.\ \phi_1(x, \ov{y}, z)$. Take any $a, b, \ov{c}$, assume $a
= b$ and $\exists z.\ \phi_1(a, \ov{c}, z)$. Then we have some $d$ such that
$\phi_1(a, \ov{c},d)$ holds. By inductive hypothesis for $\phi_1$, again
merging $\ov{y}$ with $z$, we get $\phi_1(b, \ov{c}, d)$, so also $\exists
z.\ \phi_1(b, \ov{c}, z)$ which ends the proof. 
\end{itemize}
}
{
}
\end{proof}


\ignore{
\begin{itemize}
\item $\omega$. By Lemma \ref{omegat}, it remains to show that $A \in \omega$, $A
= B$ implies $B \in \omega$. If $A \in \omega$, then $A = 0$ or there is $C
\in \omega$ such that $A = S(C)$. In the former case, $B = 0$, so $B \in
\omega$, in the latter $B = S(C)$, so $B \in \omega$ too.
\item $P(u)$. Let $D = u^T$. Take $A \in P(D) \cap T$, then $A \in T$. 
Take $B = A$. By Lemma \ref{t1}, $B \in T$ and if $c \in B$, then $c \in A$,
so $c \in D$, so $B \in P(D)$. 
\item $(SEP_\phi)$. If $a \in \{ x \in A\ |\ \phi^T(x,
\ov{B}) \}$, then $a \in A$ and $\phi^T(a, \ov{B})$, so also ${\phi^T}^T(a,
\ov{B})$. On the other hand, if $a \in A$ and ${\phi^T}^T(a, \ov{b})$, then
also $\phi^T(a, \ov{B})$, so $a \in \{ x \in A\ |\ \phi^T(x,
\ov{B}) \}$.
\item $(REPL_\phi(u, ov{u})$. Let $A = u^T$, $\ov{B} = \ov{u^T}$, by IH $A,
\ov{B} \in T$. We show that the set $C = \{ z\ |
(\forall x \in A \exists! y.\ y \in T \land \phi^T(x, y)) \land \exists x \in A.\
z \in T \land \phi^T(x, z) \}$ is in $T$. Indeed, let $a \in C$. Then
$(\forall x \in A \exists! y.\ y \in T \land \phi^T(x, y)) \land \exists x \in A.\
a \in T \land \phi^T(x, a)$. Thus $a \in T$. Now suppose $a = b$. We need to show that $b \in C$. To show that, we need
to show that $(\forall x \in A \exists! y \in T.\ \phi^T(x, y)) \land \exists x \in A.\
b \in T \land \phi^T(x, b) \}$. The first part of the conjuction is trivial. For the second
part, take $d \in A$ such that $\phi^T(d, a)$. By Lemma \ref{l3}, we also have
$\phi^T(d, b)$.
\end{itemize}
\end{proof}
}

\begin{theorem}\label{tlsmodel}
$T \models IZF$. 
\end{theorem}
\begin{proof}
\ifthenelse{\boolean{long}}
{

We proceed axiom by axiom. We have already shown the claim for (EXT) and
(L).  
\begin{itemize}

\item (PAIR) Take any $A, B \in T$. That $\{ A, B \}$ satisfies the (PAIR) axiom in T 
follows by absoluteness of equality. 
\item (UNION) Take any $A \in T$. That $\bigcup A$ satisfies its axiom in $T$ follows by
absoluteness of bounded formulas for transitive models of IZF.
\item (INF) We show that $\omega$ satisfies its respective axiom in T. Take
any $a \in T$. Obviously, if $a = 0 \lor \exists y \in T.\ y \in \omega \land \ a = S(y)$, then $a \in \omega$. 
On the other hand, suppose $a \in \omega$, then $a = 0 \lor \exists y \in
\omega.\ a = S(y)$. But since $\omega \in T$, any such
$y$ is in $T$, which gives $a = 0 \lor \exists y \in T.\ y \in \omega \land a = S(y)$
\item (POWER) First we show that for any $A \in T$, $P(A) \cap T \in T$.
Take any $B \in P(A) \cap T$. Then $B \in T$. suppose $B = C$. Then by Lemma \ref{t1}
$C \in T$ and easily $C \subseteq A$, so $C \in P(A) \cap T$. 

To show that it satisfies the (POWER) axiom, take $A \in T$, $B \in T$ and
suppose $B \in P(A) \cap T$. Then for all $b$, if $b \in B$, then $b
\in A$, so also for all $b \in T$, if $b \in B$, then $B \in A$. 

For the other direction, suppose that for all $b \in T$, if $b \in B$ then
$b \in A$. But since $B \in T$, then any element of $B$ is in $T$, so any
element of $B$ is in $A$, so $B \subseteq A$. 
\item $(SEP_\phi)$. If $a \in \{ x \in A\ |\ \phi^T(x,
\ov{B}) \}$, then $a \in A$ and $\phi^T(a, \ov{B})$, so also ${\phi^T}^T(a,
\ov{B})$. On the other hand, if $a \in A$ and ${\phi^T}^T(a, \ov{b})$, then
also $\phi^T(a, \ov{B})$, so $a \in \{ x \in A\ |\ \phi^T(x,
\ov{B}) \}$.
\item $(REPL_\phi)$. We show that the axiom is satisfied in $T$. Take any $c \in T$ such that
$c \in \{ z\ |
(\forall x \in A \exists! y.\ y \in T \land \phi^T(x, y)) \land \exists x \in A.\
z \in T \land \phi^T(x, z) \}$. Then $(\forall x \in A \exists! y.\ y \in T \land \phi^T(x, y))
\land \exists x \in A.\ c \in T \land \phi^T(x, c)$. Since $A \in T$, the
first $\forall$ and the second $\exists$ are equivalent to their
restrictions to $T$, $\exists !$ is already restricted to $T$ and
restricting of formulas to $T$ is idempotent. 
\item $(IND_\phi)$. Take $\ov{B} \in T$. Suppose that $\forall x \in T. 
(\forall y \in x.\
\phi^T(y, \ov{B})) \to \phi^T(x, \ov{B})$. We have to show that $\forall A.\ A \in T \to \phi^T(A, \ov{B})$.
We proceed by $\in$-induction on $A$. Take $A \in T$. By the assumption
instantiated with $A$, $(\forall y \in A.\ \phi^T(y, \ov{B})) \to \phi^T(A, \ov{B})$.
We have to show that $\phi^T(A, \ov{B})$. It suffices to show that $\forall
y \in A.\ \phi^T(y, \ov{B})$. But this follows immediately from the
inductive hypothesis (which is $\forall y \in A.\ y \in T \to \phi^T(y,
\ov{B})$) since $y \in A$ implies $y \in T$, by transitivity of $T$. 
\end{itemize}
}
{
Straightforward. To prove (IND) use $\in$-induction. 
}
\end{proof}

\begin{lemma}\label{tt}
IZF $\p \forall \ov{a}.\ t^T(\ov{a}) = t(\ov{a})$ and
IZF $\p \forall \ov{a}.\ \phi^T(\ov{a}) \iffl \phi(\ov{a})$.
\end{lemma}
\ifthenelse{\boolean{long}}
{
\begin{proof}
Case $t$ of:
\begin{itemize}
\item $a, \omega$. Obvious. 
\item $\{ A, B \}$. By IH, $A^T = A$ and $B^T = B$. So if $a \in \{ A^T, B^T
\}$, then $a = A$ or $a = B$, so $a \in \{ A, B \}$. The other direction is
symmetric.
\item $\bigcup A$. By IH, $A^T = A$. If $a \in \bigcup A^T$, then there is
$b$ such that $a \in b \in A^T$, so $b \in A$, so $b \in \bigcup A$. The
other direction is symmetric.
\item $P(A)$. By IH, $A^T = A$. If $a \in P(A) \cap T$, then $a \subset A$,
so $a \in P(A)$. On the other hand, if $a \in P(A)$. 
\item $\{ x \in A\ |\ \phi(x, \ov{F})$. By IH, $A^T = A, \ov{F}^T = \ov{F}$. Suppose $a \in \{ x \in A^T\ |\
\phi^T(x, \ov{F}^T) \}$. Then $a \in A^T$, so $a \in A$. Since 
$\phi^T(a, \ov{F}^T)$, since we work in IZF, $\phi^T(a, \ov{F})$. By IH, 
$\phi(a, \ov{F})$, so $a \in \{ x \in A\ |\ \phi(x, \ov{F}) \}$.
\item $\{ y\ |\ \forall x \in A\ exists !y. \phi(x, y, \ov{F}) \land \exists
x \in A.\ \phi(x, y, \ov{F}) \}$. By IH, $A^T = A, \ov{F}^T =
\ov{F}$. Suppose $a \in \{ y\ |\ \forall x \in A\ exists !y. \phi(x,
y, \ov{F}) \land \exists x \in A.\ \phi(x, y, \ov{F}) \}$. Thus:
\begin{itemize}
\item For all $x \in A$ there is exactly one $y$ such that $\phi(x,
y, \ov{F})$. Since we work in IZF, also for all $x \in A$, there is exactly
one $y \in T$ such that $\phi(x, y, \ov{F}^T)$. By IH, also
$\phi^T(x, y, \ov{F}^T)$. 
\item There is $x \in A$ such that $\phi(x, y, \ov{F})$. Again we derive
$\phi^T(x, y, \ov{F}^T)$; moreover, $V=T$ gives us $a \in T$.
\end{itemize}
Altogether, $a \in (\{ y\ |\ \forall x \in A\ exists !y. \phi(x, y, \ov{F}) \land \exists
x \in A.\ \phi(x, y, \ov{F}) \})^T$. The other direction is similar.
\end{itemize}
For the formulas, the only interesting case is atomic: $\phi \equiv t(\ov{A}) \in s(\ov{a})$. By 
Lemma \ref{tt}, $s^T(\ov{a}) = s(\ov{a})$, $t^T(\ov{a}) = t(\ov{a})$. Since
$V = T$, we get the claim.
\end{proof}
}{
\begin{proof}
By induction on the definition of terms and formulas. 
\end{proof}
}

\begin{lemma}\label{liff}
IZF $\p \phi$ iff \iizf $\p \phi^T$. 
\end{lemma}
\begin{proof}
The left-to-right direction follows by Theorem \ref{tlsmodel}, 
the right-to-left direction by Lemma \ref{tt}. 
\end{proof}

\begin{corollary}\label{dpnep}
IZF satisfies DP and NEP. 
\end{corollary}
\begin{proof}
For DP, suppose IZF $\p \phi \lor \psi$. By Lemma \ref{liff},
\iizf $\p \phi^T \lor \psi^T$. By DP for \iizf, either \iizf $\p \phi^T$ or
\iizf $\p \psi^T$. Using Lemma \ref{liff} again we get either IZF $\p \phi$ or
IZF $\p \psi$.

For NEP, suppose IZF $\p \exists x.\ x \in \omega \land \phi(x)$. By Lemma
\ref{liff}, \iizf $\p \exists x.\ x \in T \land x \in \omega^{T}.\
\phi^{T}(x)$, so \iizf $\p \exists x \in \omega^T.\ x \in T
\land  \phi^{T}(x)$. Since $\omega^{T} = \omega$, using NEP for \iizf we get
a natural number $n$ such that \iizf $\p \exists x.\ \phi^{T}(x) \land x =
\ov{n}$. By Lemma \ref{liff} and $\ov{n} = \ov{n}^T$, we get IZF $\p
\exists x.\ \phi(x) \land x = \ov{n}$. By the Leibniz axiom, IZF $\p
\phi(\ov{n})$. 
\end{proof}

We cannot establish TEP and SEP for IZF as easily, since it is not
the case that $t^T = t$ for all terms $t$ (in other words, not all
operations defined by terms are absolute with respect to $T$). However, a
simple modification to the axiomatization of IZF yields these results too. 
It suffices to guarantee that whenever a set is defined, it must be in $T$. To do this, 
we modify three axioms and add one new, axiomatizing transitive closure:
\begin{description}
\item (SEP'${}_{\phi(a, \ov{f})}$) $\forall \ov{f} \forall a \forall
c.\ c \in S_{\phi(a, \ov{f})}(a, \ov{f}) \iffl c \in a \land
\phi^T(c, \ov{f})$
\item (POWER') $\forall a \forall c. c \in P(a) \iffl c \in T \land \forall b.\ b \in c \to b \in a$
\item (REPL'${}_{\phi(a, b, \ov{f})}$) $\forall \ov{f} \forall a
\forall c. c \in R_{\phi(a, b, \ov{f})}(a, \ov{f}) \iffl
(\forall x \in a \exists! y \in T. \phi^T(x, y, \ov{f})) \land
(\exists x \in a.\ \phi^T(x, c, \ov{f}))$
\item (TC) $\forall a, c.\ c \in TC(a) \iffl c \in a \lor \exists
d \in TC(a).\ c \in d$.
\end{description}
In the modified axioms, the definition of $T$ is written using $TC$ and
relativization of formulas to $T$ this time leaves terms intact, we set $t^T \equiv
t$ for all terms $t$. It is not difficult to see that this axiomatization is equivalent to the old
one. We can therefore adopt it as the official axiomatization of IZF. All the developments 
in sections 4-8 can be done for the new axiomatization in the similar way and in the end we get:
\begin{corollary}\label{dpneptepsep}
IZF satisfies DP, NEP, TEP and SEP. 
\end{corollary}
\begin{proof}
DP and NEP follow in the same way as in Theorem \ref{dpnep}. For TEP,
if IZF $\p \exists x.\ \phi(x)$, then IZF${}^{-}$ $\p \exists x \in T.\
\phi^T(x)$, so there is a term $t$ such that IZF${}^{-}$ $\p t \in T \land
\phi^T(t)$, so since $t^T = t$, IZF $\p \phi(t)$. To prove SEP proceed as
in Corollary \ref{sep}. 
\end{proof}


==> model.tex <==
\section{Model}

Here we explain the metalevel definitions using a model of IZF. 

We work in IZF with inaccessible cardinal. There is a transitive model $I$
of IZF in our universe. In $I$, there is a class of lambda names,
$I^\lambda$. Lambda terms are absolute, so is the reduction relation,
natural numbers, so $M \downarrow v$ iff $I \models M \downarrow v$. 

First we define relation $(M, \rho) \reals \phi$, for $M \in \Lambda$, $\rho
: Var \to I^\lambda$, and for $\phi$ in a standard language and along with
it, a formula $\phi^*$ of IZF. Any such $\rho$ is an object in $M$, as
a finite function. We prove on the way that $(M, \rho) \reals
\phi$ iff $I, q:=\rho \models \phi^*(M)$. We do it by induction on $\phi$. Case $\phi$ of:
\begin{itemize}
\item $a \in b$. This means that $M \downarrow v$ and $(v, \rho(a)) \in
\rho(b)$. $\phi^* \equiv M \downarrow v \land (v, q(a)) \in q(b)$.
Suppose $M \downarrow v$ and $(v, \rho(a)) \in \rho(b)$. 
Then $I, q:=\rho \models M \downarrow v$ and $I, q :=\rho \models (v, q(a))
\in q(b)$. OTOH, suppose $I, q:=\rho \models M \downarrow v and (v, (q(a))
\in q(b)$. Then $M \downarrow v$ and $(v, \rho(a)) \in \rho(b)$. 
\item $\forall a.\ \phi$. This means that for all $A \in I^\lambda$,
$(M, \rho[a:=A]) \reals \phi$. $\phi^* \equiv \forall a \in I^\lambda.\
\phi^*$. Suppose for all $A \in I^\lambda$,
$(M, \rho[a:=A]) \reals \phi$. By IH, iff for ll $A \in
I^\lambda$, $I, \rho[a:=A] \models \phi^*$. Iff $I \models \forall a \in
I^\lambda.\ \phi^*$.
\end{itemize}

\begin{lemma}
For all $\phi$, for all $M, \rho$, if $(M, \rho) \reals \phi$ then $M \downarrow$. 
\end{lemma}
\begin{proof}
Induction on $\phi$. For atomic case it's obvious, for $\forall a.\ \psi$,
$M \reals_\rho \forall a.\ \psi$ iff $\forall A \in I^\lambda, (M,
\rho[a:=A]) \reals \phi$. Take any $A \in I^\lambda$, by IH $M \downarrow$.
\end{proof}

\begin{lemma}
For all $\phi$, If $M \to M'$ then $M \reals_rho \phi$ iff $M' \reals_\rho \phi$. 
\end{lemma}
\begin{proof}
Induction on $\phi$. For the atomic case, assume $M \to M'$. If $M
\reals_\rho \phi$, then $M \downarrow to v$ and $(v, A) \in B$. So also $M'
\downarrow v$ and $(v, A) \in B$. On the other hand, the argument works the
same. For $\forall a.\ \phi$, if $M \to M'$ then for all $A$, $M \reals
\phi$, so $M' \reals \phi$, so $M' \reals \forall a.\ \phi$. 
\end{proof}

The lemmas relating ranks to sets work as usual $M \reals A \in B$. 

Now, the meaning of a term. Let's do separation.
\[
Q = \SB{\{ x \ |\ \phi(x) \}} = \{ (sepRep(N), A) \in I\ |\ I, \rho[x:=A] \models \phi^*(N) \}
\]
First, let's note that $Q \in I^\lambda$, by rank considerations and the
validity of appropriate axioms in $I$. Its definition is $\{ sepRep(N), A)\
|\ \phi*(N) \}$. Suppose $(M, A) \in Q$. Then $(M = sepRep(N)$ and $I,
\rho[x:=A] \models \phi^*(N)$. This means that $N \reals_{\rho[x:=A]} \phi$.
On the other hand, suppose $N \reals_{\rho[x:=A]} \phi$. Then $I, \rho[x:=A]
\modles \phi^*N()$, so $


==> omegaizf.tex <==
\begin{lemma}\label{lreal1}
For any $A$, $<I, I> \reals_\rho A = A$. 
\end{lemma}
\begin{proof}
$<I, I> \reals_\rho A = A$ means $<I, I> \reals_\rho \forall b.\ b\ in A
\iffl b \in A$ which is $<I, I> \reals_\rho (\forall b.\ b\ in A
\to b \in A) \land (\forall b.\ b\ in A
\to b \in A)$. It suffices to show that $I \reals_\rho \forall b.\ b\ in A
\to b \in A$. That is, that for all $B$, $M$, if $M \reals B \in A$ then $I\
M \reals B \in A$. But $I M \downarrow M$, so the claim trivially follows. 
\end{proof}

\begin{lemma}\label{lreal2}
If $(M, A) \in \omega$, then $M \reals_\rho A \in \omega$.
\end{lemma}
\begin{proof}
A trivial proof by induction on the definition of $\omega$ --- all that's to
show is that $M$ is in a normal form, which follows immediately. 
\end{proof}

\begin{lemma}
If $M \reals_\rho A \in \omega$, then $M \reals_\rho A = 0 \lor \exists y.\ y \in
\omega \land A = S(y)$. 
\end{lemma}
\begin{proof}
Suppose $M \reals_\rho A \in \omega$. Then $M \downarrow v$ and $(v, A) \in
\omega$. We proceed by induction on the definition of $\omega$:
\begin{itemize}
\item Base case. Then $v = natRep(<inl(<I, I>))$ and $A = 0$. We need to
show that $<inl(<I, I>) \reals_\rho 0 = 0 \lor \exists y.\ y \in \omega \land y = S(0)$.
To show this, all we need to show that $<I, I> \reals_\rho 0 = 0$ which
holds by Lemma\ref{lreal1}.
\item Inductive case. Then $v = natRep((inr(<N, <I, I>)))$, where $(N, D)
D \in \omega$, for $A = S(D)$. Thus also, by Lemma \ref{lreal2}, $N
\reals_\rho D \in \omega$. 
We need to show that $inr(<N, <I, I>) \reals
A = 0 \lor \exists y.\ y \in \omega \land A = S(y)$, that is that
$<N, <I, I> \reals \exists y.\ y \in \omega \land A = S(y)$, that is that
there is $B$ such that $<N, <I, I>> \reals B \in \omega \land A = S(B)$. 
Take $B=D$. The claim easily follows. 
\end{itemize}
\end{proof}


==> realnorm.tex <==
\section{Weak normalization for simply-typed lambda calculus}
\begin{definition}
The terms of simply-typed lambda calculus are generated by the following
grammar:
\[
M ::= x\ |\ \lambda x.\ M\ |\ M\ N\ |\ magic(M)
\]
\end{definition}
\begin{definition}
The types (formulas) are generated by the following grammar:
\[
\tau ::= \bot\ |\ \tau \to \tau\ |\ a
\]
\end{definition}
where $a$ is a variable, coming from a designated set of type variables. We
call a type \emph{atomic} if it is not an arrow type.
\begin{definition}
The typing rules are as follows, where $\Gamma$ is a context, containing a
list of pairs of the form $(x, \tau)$, where $x$ is a variable and $\tau$ is
a type:
\[
\infer{\gxp x : \tau}{} \qquad \infer{\gp \lambda x : \sigma.\ M : \sigma
\to \tau}{\gxp M : \tau} \qquad \infer{\gp M\ N : \tau}{\gp M : \sigma \to
\tau & \gp N : \sigma} \qquad \infer{\gp magic(M) : \tau}{\gp M : \bot}
\]
\end{definition}
\begin{definition}
The deduction rules result from the typing rules by erasure of lambda terms:
\[
\infer{\g, \tau \p \tau}{} \qquad \infer{\gp \sigma
\to \tau}{\gamma, \sigma \proves \tau} \qquad \infer{\gp \tau}{\gp \sigma \to
\tau & \gp \sigma} \qquad \infer{\gp \tau}{\gp \bot}
\]
\end{definition}
\begin{definition}
The calculus is call-by-name. That is, the only reduction rule is:
\[
(\lambda x : \tau.\ M)\ N \to M[x:=N]
\]
\end{definition}
\begin{definition}
We designate certain lambda terms as \emph{values}. Namely, the values are
lambda-abstractions. 
\end{definition}

\begin{definition}
By induction on the type structure we define a realizability relation $\real$ between lambda-terms
and types in the following way:
\begin{itemize}
\item (Base case 1) For no term $M$ it is the case that $M \real \bot$.
\item (Base case 2) For no term $M$ it is the case that $M \real a$, where
$a$ is a type variable.
\item (Inductive step) $M \real \sigma \to \tau$ if $M \downarrow \lambda x
: \sigma. Q$ and forall $N$, if $N \real \sigma$, then $Q[x:=N] \real \tau$. 
\end{itemize}
\end{definition}
\begin{lemma}\label{reall1}
If $M \to O$, then $M \real \tau$ iff $O \real \tau$, for all types $\tau$. 
\end{lemma}
\begin{proof}
By induction on $\tau$. For atomic types the claim is obvious. Suppose $M
\real \sigma \to \tau$ and $M \to O$. Then $M \downarrow \lambda x : \sigma
N$ and forall $Q$, if $Q \real \sigma$, then $N[x:=Q] \real \tau$. Obviously $O
\downarrow \lambda x : \sigma.\ N$ as well so the claim about $Q$ is going
to be satisfied as well. 

Now suppose $O \real \tau$ and $M \to O$. Then $O \downarrow
\lambda x : \sigma.\ N$ and so does $M$. Again, the claim about $Q$ is
trivial. 
\end{proof}
\begin{definition}
Let $\rho$ be a function from variables to lambda-terms and let $\Gamma$ be
an environment. We write $\Gamma \models \rho$ if for all $(x, \tau) \in
\Gamma$, $\rho(x) \real \tau$. We write $M[\rho]$ to denote a lambda-term
resulting from $M$ by substituting $\rho(x)$ for any free variable $x$ of
$M$. 
\end{definition}
We assume some way to assign a typing context $\ov{\g}$ to any logic
context $\g$, for example to a context $a, b$ there can correspond a context
$x_1 : a, x_2 : b$.
\begin{theorem}\label{realt1}
If $\gp \tau$, then there is a term $M$ such that $\ov{\g} \proves M : \tau$ 
and for any $\rho$ such that $\ov{\g} \models \rho$, $M[\rho]
\real \tau$. 
\end{theorem}
\begin{proof}

By induction on the proof of $\Gamma \proves \tau$. Case $\Gamma \proves \tau$ of:
\begin{itemize}
\item $\infer{\Gamma, \tau \proves \tau}{}$. Then $\infer{\ov{\g}, x : \tau \proves
x : \tau}{}$. Take any $\rho$ such that $\ov{\g}, x : \tau \models \rho$,
then $\rho(x) \real \tau$, so $x[\rho] = \rho(x) \real \tau$. 
\item $\infer{\gp \tau}{\gp \sigma \to \tau & \gp \sigma}$. 
By IH, for any $\rho \models \ov{\g}$, we get $M, N$ such that:
\begin{itemize}
\item $\ogp M : \sigma \to \tau$
\item $\ogp N : \sigma$
\item $M[\rho] \real \sigma \to \tau$
\item $N[\rho] \real \sigma$
\end{itemize}
Then $\ogp M\ N : \tau$. Moreover, since $M[\rho] \real \sigma \to \tau$,
then $M[\rho] \downarrow \lambda x : \sigma.\ P$ for some $P$ and
$P[x:=N[\rho]] \real \tau$. Since $(M\ N)[\rho] = M[\rho]\ N[\rho] \to^*
(\lambda x : \sigma.\ P)\ N[\rho] \to P[x:=N[\rho]]$, Lemma \ref{reall1}
applied the correct number of times gives us that $(M\ N)[\rho] \real \sigma
\to \tau$. 
\item $\infer{\gp \sigma \to \tau}{\g, \sigma \p \tau}$. By IH we get $M$
such that $\ov{\g}, x : \sigma \p M : \tau$ and for any $\rho \models
\ov{\g, \sigma}$, $M[\rho] \real \tau$. Therefore $\ogp \lambda x : \sigma.\  M :
\tau$. Take any $\rho$ such that $\ov{\g} \models \rho$. We have (after
appropriate choosing of $x$, so that $x \notin dom(\rho)$ ) $(\lambda x : \sigma.\ M)[\rho] = \lambda x :
\sigma. M[\rho] \downarrow \lambda
x : \sigma.\ M[\rho]$. So all we need to show is that for any $Q \real \sigma$,
$M[\rho][x:=Q] \real \tau$. Let $\rho' = \rho \cup \{ (x, Q) \}$. Then 
$M[\rho][x:=Q] = M[\rho']$, $\ov{\g, \sigma} \models \rho'$, so $M[\rho'] =
M[\rho][x:=Q] \real \tau$. This ends the proof.
\item $\infer{\gp \tau}{\gp \bot}$. By IH we get $M$ such that:
\begin{itemize}
\item $\ogp M : \bot$.
\item For any $\rho$ such that $\og \models \rho$, $M[\rho] \real \bot$.
However, this actually means that there isn't any $\rho$ such that $\og
\models \rho$. 
\end{itemize}
Therefore $\ogp magic(M) : \tau$. The claim about the realizability is
trivial. 
\end{itemize}
\end{proof}
\begin{theorem}
If $\proves \tau$ for non-atomic $\tau$, then there is $M$ such that $\proves M : \tau$ and $M
\downarrow$. 
\end{theorem}
\begin{proof}
We take $M$ from the previous theorem, since it's easy to see that $M$ must
be closed, we get $M \real \tau$, since $\tau$ is non-atomic, then it is an
arrow type, so $M \downarrow \lambda x : \tau_1. Q$. 
\end{proof}



==> redla.tex <==
\subsection{Reduction rules}\label{rr}

The reduction relation $\to$ arises by lazily evaluating the
following reduction rules. 

\[
(\lambda x. M) N \to M[x:=N]
\]
\[
fst(<M, N>) \to M
\]
\[
snd(<M, N>) \to N
\]
\[
case(inl\ M, x.N, x.O) \to N[x:=M]
\]
\[
case(inr\ M, x.N, x.O) \to O[x:=M]
\]
\[
axiomProp(axiomRep(M)) \to M \qquad \mbox{ for axiom in pair/$sep_{\phi}$}
\]



==> selfap.tex <==
\section{Self application in non-well-founded set theory}

We present an example of self-applicating proof in non-well-founded set
theory. The example is based on Crabbe's counterexample showing that
standard set theory doesn't enjoy cut elimination property. 

Consider a set theory in an intuitionistic first order logic \emph{without} equality 
with one relational symbol $\in$, two constants C, D and the following axioms, where $a=b$ is a metalevel abbreviation for
$\forall x.\ x \in a \iffl x \in b$. 

\begin{itemize}
\item (NWF) $\forall a.\ a\ \in C \iffl a = C$
\item (SEP0) $\forall a.\ a \in D \iffl a \in C \land (a \in a \to a \in a)$
\end{itemize}

The (NWF) axiom expresses that $C$ is a non-well founded set, $C= \{ C \} $. The (SEP1) is
an instance of a full separation axiom --- $D$ traditionally would be displayed as
$\{ x \in C\ |\ x \in x \to x \in x \}$. This theory is consistent. 

\begin{lemma}\label{l0}
$D=C$.
\end{lemma}
\begin{proof}
If $a \in D$, then obviously $a \in C$. On the other hand, if $a \in C$,
then trivially $a \in a \to a \in a$, so also $a \in D$. 
\end{proof}

\begin{lemma}\label{l05}
$D \in C$. 
\end{lemma}
\begin{proof}
Note --- this \emph{does not} follow trivially from Lemma \ref{l0}, since we
do not have the Leibniz axiom. However, by (NWF) we get the claim. 
\end{proof}

\begin{lemma}\label{l1}
If $D \in D$ then $D \in D$. 
\end{lemma}
\begin{proof}
Of course trivial, but we will prove the claim in a bit more
convoluted way. Suppose $D \in D$. Then by (SEP0), $D \in D \to D \in D$. 
Thus, by applying this implication to our assumption, we get $D \in D$. 
\end{proof}

\begin{lemma}\label{l2}
$D \in D$. 
\end{lemma}
\begin{proof}
Trivial again by Lemmas \ref{l0}, \ref{l05} and again we'll do the proof in a more
convoluted way. By Lemma \ref{l1}, $D \in D \to D \in D$. By Lemma \ref{l05}, 
$D \in C$, so by (SEP0) $D \in D$. By Lemma \ref{l1} therefore, $D \in D$. 
\end{proof}

The proof of Lemma \ref{l2} is as bizarre as you can get. In the proof, Lemma
\ref{l1} is applied to itself. This cannot be left unpunished, and
indeed, the resulting proof term in a corresponding lambda calculus doesn't
even weakly normalize, as shown below.

The non-well-foundedness is not as essential as it seems, it is possible
to construct a similar proof (which weakly normalizes, though) in a 
$ZF^{-}$ set theory. $C$ then becomes a variable and an assumption $D \in C$
(false in ZF) needs to be added to Lemma \ref{l2}. 

\subsection{Non-normalising proof}

Let $nRep, nProp, sRep, sProp$ denote the rep and prop
terms for $(NWF)$ and $(SEP0)$ respectively.
The proof tree $T_{\ref{l0}}$ for the Lemma \ref{l0} is as follows.
\[
\infer
{
\p \lambda a.\ <\lambda x : a \in D.\ fst(sProp(x)), \lambda x : a \in C.\
sRep(<x, \lambda y : a \in a. y>)> : \forall a.\ (a \in D \to a \in C \land
a \in C \to a \in D)
}
{
 \infer
 {
 \p <\lambda x : a \in D.\ fst(sProp(x)), \lambda x : a \in C.\
 sRep(<x, \lambda y : a \in a. y>)> : (a \in D \to a \in C \land
 a \in C \to a \in D)
 }
 {
   \infer
   {
   \p \lambda x : a \in D.\ fst(sProp(x)) : a \in D \to a \in C
   }
   {
     \infer
     {
       x : a \in D \p fst(sProp(x)) : a \in C
     }
     {
       \infer{x : a \in D \p sProp(x) : a \in C \land (a \in a \to a \in a)}
             {\infer{x : a \in D \p x : a \in D}{}}
     }
   }
   &
   \infer
   {
     \p \lambda x : a \in C.\ sRep(<x, \lambda y : a \in a. y>) : a \in C \to a \in D
   }
   {
     \infer
     {
       x : a \in C \p sRep(<x, \lambda y : a \in a. y>) : a \in D
     }
     {
       \infer
       {
         x : a \in C \p <x, \lambda y : a \in a. y> : a \in C \land a \in a \to a \in a
       }
       {
         \infer{
	   x : a \in C \p x : a \in C
	 }
	 {}
	 &
	 \infer 
	 {
	   x : a \in C \p \lambda y : a \in a. y : a \in a \to a \in a
	 }
	 {
	   \infer{x : a \in C, y : a \in a \p y : a \in a}{}
	 }
       }
     }
   }
 }
}
\]

Let $M_{\ref{l0}}$ denote the respective proof term. 

The proof tree $T_{\ref{l05}}$ for Lemma \ref{l05} is as follows:
\[
\infer{\p nRep(M_{\ref{l0}}) : D \in C}{
\infer{\p M_{\ref{l0}} : D = C}{T_{\ref{l0}}}}
\]

Let $M_{\ref{l05}}$ denote the respective proof term. 

The proof tree $T_{\ref{l1}}$ along with the respective proof term
$M_{\ref{l1}}$ is as follows:

\[
\infer
{
\p \lambda x : D \in D.\ snd(sProp(x))\ x : D \in D \to D \in D
}
{
  \infer
  {
  x : D \in D \p snd(sProp(x))\ x : D \in D
  }
  {
      \infer
      {
        x : D \in D \p snd(sProp(x)) : D \in D \to D \in D
      }
      {
        \infer
	{
	  x : D \in D \p sProp(x) : D \in D \land (D \in D \to D \in D)
	}
	{
	  \infer{x : D \in D \p x : D \in D}{}
	}
      }
      &
      \infer{ x : D \in D \p x : D \in D}{}
  }
}
\]

Finally, the proof tree $T_{\ref{l2}}$ along with the respective proof term
$M_{\ref{l2}}$ is as follows:
\[
\infer
{
\p M_{\ref{l1}}\ sRep(<M_{\ref{l05}}, M_{\ref{l1}}>) : D \in D
}
{
  \infer{\p M_{\ref{l1}} : D \in D \to D \in D}{T_{\ref{l1}}}
  &
  \infer{\p sRep(<M_{\ref{l05}}, M_{\ref{l1}}>) : D \in D}
  {
    \infer{\p <M_{\ref{l05}}, M_{\ref{l1}}> : D \in D \land (D \in D \to D \in D)}
    {
      \infer{\p M_{\ref{l05}} : D \in D}{T_{\ref{l05}}}
      &
      \infer{\p M_{\ref{l1}} : D \in D \to D \in D}{T_{\ref{l1}}}
    }
  }
}
\]

Finally, the nonterminating computation:
\[
M_{\ref{l1}}\ (sRep(<M_{\ref{l05}}, M_{\ref{l1}}>)) = (\lambda x : D \in D.\
snd(sProp(x))\ x)\ (sRep(<M_{\ref{l05}}, M_{\ref{l1}}>) \to
snd(sProp(sRep(<M_{\ref{l05}}, M_{\ref{l1}}>)))\ (sRep(<M_{\ref{l05}},
M_{\ref{l1}}>)) \to 
\]
\[
\to snd(<M_{\ref{l05}}, M_{\ref{l1}}>))\ (sRep(<M_{\ref{l05}},
M_{\ref{l1}}>) \to M_{\ref{l1}}\ (sRep(<M_{\ref{l05}}, M_{\ref{l1}}>) \to {\ldots}
\]

An interesting questions is whether it is possible to get a non-normalizing proof term without
(NWF). 


==> selfap1.tex <==
\section{Self application in non-well-founded set theory}

We present an example of self-applicating proof in non-well-founded set
theory. The example is based on Crabbe's counterexample showing that
standard set theory doesn't enjoy cut elimination property. 

Consider a set theory in an intuitionistic first order logic without equality
with one relational symbol $\in$, two constants C, D and the following axioms, where $a=b$ is a metalevel abbreviation for
$\forall x.\ x \in a \iffl x \in b$. 

\begin{itemize}
\item (NWF) $\forall a.\ a\ \in C \iffl a = C$
\item (SEP0) $\forall a.\ a \in D \iffl a \in C \land (a \in a \to a \in C)$
\end{itemize}

The (NWF) axiom expresses that $C$ is a non-well founded set, $C= \{ C \} $. The (SEP1) is
an instance of a full separation axiom --- $D$ traditionally would be displayed as
$\{ x \in C\ |\ x \in x \to x \in C \}$. This theory is consistent. 

\begin{lemma}\label{l0}
$D=C$.
\end{lemma}
\begin{proof}
If $a \in D$, then obviously $a \in C$. On the other hand, if $a \in C$,
then trivially $a \in a \to a \in C$, so also $a \in D$. 
\end{proof}

\begin{lemma}\label{l05}
$D \in C$. 
\end{lemma}
\begin{proof}
Note --- this \emph{does not} follow trivially from Lemma \ref{l0}, since we
do not have the Leibniz axiom. However, by (NWF) we get the claim. 
\end{proof}

\begin{lemma}\label{l1}
If $D \in D$ then $D \in C$.
\end{lemma}
\begin{proof}
Of course trivial, but we will prove the claim in a bit more
convoluted way. Suppose $D \in D$. Then by (SEP0), $D \in D \to D \in C$. 
Thus, by applying this implication to our assumption, we get $D \in C$.
\end{proof}

\begin{lemma}\label{l2}
$D \in C$. 
\end{lemma}
\begin{proof}
Trivial again by Lemma \ref{l05} and again we'll do the proof in a more
convoluted way. By Lemma \ref{l1}, $D \in D \to D \in C$. By Lemma \ref{l05}, 
$D \in C$, so by (SEP0) $D \in D$. By Lemma \ref{l1} therefore, $D \in C$.
\end{proof}

The proof of Lemma \ref{l2} is as bizarre as you can get. In the proof, Lemma
\ref{l1} is applied to itself. This cannot be left unpunished, and
indeed, the resulting proof term in a corresponding lambda calculus doesn't
even weakly normalize, as shown below.

The non-well-foundedness is not as essential as it seems, it is possible
to construct a similar proof (which weakly normalizes, though) in a 
$ZF^{-}$ set theory. $C$ then becomes a variable and an assumption $D \in C$
(false in ZF) needs to be added to Lemma \ref{l2}. 

\subsection{Non-normalising proof}

Let $nRep, nProp, sRep, sProp$ denote the rep and prop
terms for $(NWF)$ and $(SEP0)$ respectively.
The proof tree $T_{\ref{l0}}$ for the Lemma \ref{l0} is as follows.
\[
\infer
{
\p \lambda a.\ <\lambda x : a \in D.\ fst(sProp(x)), \lambda x : a \in C.\
sRep(<x, \lambda y : a \in a. y>)> : \forall a.\ (a \in D \to a \in C \land
a \in C \to a \in D)
}
{
 \infer
 {
 \p <\lambda x : a \in D.\ fst(sProp(x)), \lambda x : a \in C.\
 sRep(<x, \lambda y : a \in a. y>)> : (a \in D \to a \in C \land
 a \in C \to a \in D)
 }
 {
   \infer
   {
   \p \lambda x : a \in D.\ fst(sProp(x)) : a \in D \to a \in C
   }
   {
     \infer
     {
       x : a \in D \p fst(sProp(x)) : a \in C
     }
     {
       \infer{x : a \in D \p sProp(x) : a \in C \land (a \in a \to a \in a)}
             {\infer{x : a \in D \p x : a \in D}{}}
     }
   }
   &
   \infer
   {
     \p \lambda x : a \in C.\ sRep(<x, \lambda y : a \in a. y>) : a \in C \to a \in D
   }
   {
     \infer
     {
       x : a \in C \p sRep(<x, \lambda y : a \in a. y>) : a \in D
     }
     {
       \infer
       {
         x : a \in C \p <x, \lambda y : a \in a. y> : a \in C \land a \in a \to a \in a
       }
       {
         \infer{
	   x : a \in C \p x : a \in C
	 }
	 {}
	 &
	 \infer 
	 {
	   x : a \in C \p \lambda y : a \in a. y : a \in a \to a \in a
	 }
	 {
	   \infer{x : a \in C, y : a \in a \p y : a \in a}{}
	 }
       }
     }
   }
 }
}
\]

Let $M_{\ref{l0}}$ denote the respective proof term. 

The proof tree $T_{\ref{l05}}$ for Lemma \ref{l05} is as follows:
\[
\infer{\p nRep(M_{\ref{l0}}) : D \in C}{
\infer{\p M_{\ref{l0}} : D = C}{T_{\ref{l0}}}}
\]

Let $M_{\ref{l05}}$ denote the respective proof term. 

The proof tree $T_{\ref{l1}}$ along with the respective proof term
$M_{\ref{l1}}$ is as follows:

\[
\infer
{
\p \lambda x : D \in D.\ snd(sProp(x))\ x : D \in D \to D \in D
}
{
  \infer
  {
  x : D \in D \p snd(sProp(x))\ x : D \in D
  }
  {
      \infer
      {
        x : D \in D \p snd(sProp(x)) : D \in D \to D \in D
      }
      {
        \infer
	{
	  x : D \in D \p sProp(x) : D \in D \land (D \in D \to D \in D)
	}
	{
	  \infer{x : D \in D \p x : D \in D}{}
	}
      }
      &
      \infer{ x : D \in D \p x : D \in D}{}
  }
}
\]

Finally, the proof tree $T_{\ref{l2}}$ along with the respective proof term
$M_{\ref{l2}}$ is as follows:
\[
\infer
{
\p M_{\ref{l1}}\ sRep(<M_{\ref{l05}}, M_{\ref{l1}}>) : D \in D
}
{
  \infer{\p M_{\ref{l1}} : D \in D \to D \in D}{T_{\ref{l1}}}
  &
  \infer{\p sRep(<M_{\ref{l05}}, M_{\ref{l1}}>) : D \in D}
  {
    \infer{\p <M_{\ref{l05}}, M_{\ref{l1}}> : D \in D \land (D \in D \to D \in D)}
    {
      \infer{\p M_{\ref{l05}} : D \in D}{T_{\ref{l05}}}
      &
      \infer{\p M_{\ref{l1}} : D \in D \to D \in D}{T_{\ref{l1}}}
    }
  }
}
\]

Finally, the nonterminating computation:
\[
M_{\ref{l1}}\ (sRep(<M_{\ref{l05}}, M_{\ref{l1}}>)) = (\lambda x : D \in D.\
snd(sProp(x))\ x)\ (sRep(<M_{\ref{l05}}, M_{\ref{l1}}>) \to
snd(sProp(sRep(<M_{\ref{l05}}, M_{\ref{l1}}>)))\ (sRep(<M_{\ref{l05}},
M_{\ref{l1}}>)) \to 
\]
\[
\to snd(<M_{\ref{l05}}, M_{\ref{l1}}>))\ (sRep(<M_{\ref{l05}},
M_{\ref{l1}}>) \to M_{\ref{l1}}\ (sRep(<M_{\ref{l05}}, M_{\ref{l1}}>) \to {\ldots}
\]

An interesting questions is whether it is possible to get a non-normalizing proof term without
(NWF). 


==> setizf.tex <==
\section{Relations between sets and types}

We show several relations between IZF sets and types.

Our lambda calculus is at the same time Church and Curry --- we have both
typed and untyped lambda-abstractions, with standard typing rules for
whatever type system we consider. A lambda term is \emph{annotated} if
every lambda abstraction is typed. 

We are going to consider various formal set theories. Any of them is strong
enough to formalize arithmetic and provability predicate $Pr$. We need the
following two theorems, where $T$ is the theory considered. 

\begin{theorem}
For $\Sigma_1$-sentence $\phi$, $T \proves \phi \to Pr_T(\phi)$. 
\end{theorem}
\begin{proof}
This is $\Sigma_1$-completeness of $T$, we even have $PA \proves \phi \to
\Pr_T(\phi)$,. 
\end{proof}
\begin{theorem}
For $\Sigma_1$-sentence $\phi$, if $T \proves Pr_T(\phi)$ then $T \proves
\phi$. 
\end{theorem}
\begin{proof}
$T \proves Pr_T(\phi)$ means that for some natural number $n$, $T$ shows
that $n$ codes this proof. 
\end{proof}

Lambda terms, since they are finite objects, are absolute, so we have them
both on the meta-level and inside of the set theory, encoded as natural
numbers, for example. Moreover, the sentence ``$M \downarrow v$'' is
$\Sigma^0_1$ --- there exists a sequence encoding the reduction sequence
starting with $M$ and ending with $v$. Therefore it's absolute as well. So
is the sentence ``$M \downarrow$'', for the same reasons. Any standard
theorems about lambda-terms --- subject reduction, progress, preservation
are $\Sigma^0_1$ as well. 

\section{Set theories}

The set theories (CZF/IZF) we consider are always theories with equality and
one relation symbol $\in$. However, it's much more convenient to have set
theories with terms. Thus, we think of the theories as having terms $t$ for
any provable sentence $\exists! x.\ \phi(x)$. However, any statement
involving these terms should be treated as a metalevel abbreviation for the
sentence resulting from unwinding all the definitions.

Suppose $M \reals \exists !x.\ \phi(x)$. This means that $M \reals \exists
x.\ \phi(x) \land \forall y.\ \phi(y) \to \phi(x)$. This means that $\exists
A.\ M \reals \phi(A) \land \forall y.\ \phi(y) \to \phi(A)$. So $\exists A.\
M \downarrow <M_0, M_1> \land M_0 \reals \phi(A) \land M_1 \reals \forall
y.\ \phi(y) \to \phi(A)$. Therefore $\exists A.\ M \downarrow <M_0, M_1>
\land (M_0 \reals \phi(A)) \land \forall B.\ M_1 \reals \phi(B) \to \phi(A)$. 



\section{Realizability}

\begin{definition}[IZF]
A $\lambda$-name is a set, whose elements are hereditarily labelled by
lambda-terms. That is, if $A$ is a $\lambda$-name iff all its elements are
pair $(M, B)$ such that $M$ is a lambda-terms and $B$ is a $\lambda$-name. 
\end{definition}

\begin{definition}
The class of $\lambda$-names is denoted by $V^{\lambda}$.
\end{definition}

\begin{definition}
For any $\lambda$-name $A$, we denote by $A^0$ the set corresponding to $A$
after erasing all labels.
\end{definition}

\begin{definition}
To define the notion of realizability in the universe of IZF, we first
define a language $L$. The language is first-order, class-sized, with constants for all
$\lambda$-names. 
\end{definition}
What it means is that the language is definable in the IZF universe, i.e. we
have a formula $\phi(x)$ saying ``$x$ is a formula of $L$'', another one
$\psi(x, y, z)$ saying ``$x$
is a formula $A \in B$ of $L$ and $y$ is $A$ and $z$ is $B$'' and so one. 

Now we define the notion of realizability. We say under what circumstances
$M \reals \phi$ for $\phi \in L$. Contrary to the appearance, this relation
\emph{is not} defined by induction on $\phi$. At least in the universe. This
is because there is nothing to do induction on in the universe --- since
formulas are not sets, but classes. 

Here comes the definition (in IZF). All quantifiers quantify over
$V^\lambda$. 

\begin{itemize}
\item $M \reals A \in B$ iff $A^0 \in B^0$, $M \downarrow <M_1, M_2>$ and there is $C$ such that 
$M_1 \reals A = C$ and $(M_2, C) \in B$.
\item $M \reals A = B$ iff $A^0 = B^0$ and $M \downarrow <M_1, M_2>$ and $M_1 \downarrow
\lambda x. M_{11}$ and $M_2 \downarrow \lambda x. M_{12}$ and for all $N,
C$, if $(N, C) \in A$ then $M_{11}[x:=N] \reals C \in B$ and if $(N, C) \in
B$, then $M_{12}[x:=N] \reals C \in A$. 
\item $M \reals \phi \land \psi$ iff $M \downarrow <M_1, M_2>$ and $M_1
\reals \phi$ and $M_2 \reals \psi$. 
\item $M \reals \phi \lor \psi$ iff either $M \downarrow inl\ M_1$ and $M_1
\reals \phi$ or $M \downarrow inl\ M_2$ and $M_2 \reals \psi$. 
\item $M \reals \phi \to \psi$ iff $\phi^0 \to \psi^0$ and $M \downarrow \lambda x. M_1$ and for all
$N \reals \phi$, $M_1[x:=N] \reals \psi$.
\item $M \reals \forall a.\ \phi$ iff for all $A$, $M \reals \phi[a:=A]$.
\item $M \reals \exists a.\ \phi$ iff there is $A$ such that $M \reals
phi[a:=A]$.
\end{itemize}

This definition certainly \emph{looks} like it was defined by induction on
$\phi$. In a way it is, but on a metalevel, unwinding $\phi$ and resorting
to transfinite induction for atomic formulas. For example, the formula $M
\reals \forall x, y.\ x = y \land x \in y$ unwinds to $\forall x, y. M 
\downarrow <M_1, M_2> \land M_1 \reals x = y \land x \in y$ which unwinds to
$\forall x, y. M \downarrow <M_1, M_2> \land M_1 \downarrow <M_{11}, M_{12}>
\land M_{11} \reals x = y \land M_{12} \reals x \in y$ where the atomic
clauses are defined by simultaneous induction on $\in$.

\begin{theorem}\label{lir}[HA]
If $IZF \proves \phi$, then there is $M$ such that $IZF \proves M \real \phi$.
\end{theorem}
\begin{proof}
McCarty, Rathjen. Induction on $\phi$. 
\end{proof}
\begin{theorem}[HA]
For any $\phi \in L$ and $M$, $IZF \proves (M \real \phi) \to \phi^0$. 
\end{theorem}
\begin{proof}
By metalevel induction on $\phi$. Case $\phi$ of:
\begin{itemize}
\item $A \in B$. Then $M \reals \phi$ includes a clause $A^0 \in B^0$.
\item $A = B$. Then $M \reals \phi$ includes a clause $A^0 = B^0$.
\item $\phi \land \psi$. Then $M \real \phi \land \psi$ \emph{is} really $M
\downarrow <M_0, M_1>$ and $M_0 \reals \phi$ and $M_1 \reals \psi$, hence we
get the claim by inductive hypothesis.
\item $\phi \lor \psi$. Then $M \real \phi \lor \psi$ is ``($M
\downarrow inl(M_1)$ and $M_1 \reals \phi$) or ($M \downarrow inr(M_1)$ and
$M_1 \reals \psi$)''. So also $M_1 \reals \phi$ or $M_1 \reals \psi$. Since
by IH $M_1 \reals \phi$ implies $\phi^0$ and the same happens with $\psi$,
we get the claim. 
\item $\phi \to \psi$. Immediate.
\item $\forall a. \phi(a)$. Suppose $M \real \forall a.\ \phi(a)$. We need
to show that $(\forall a.\ \phi(a))^0$, that is $\forall c.\ \phi^0[a:=c]$.
So take any $C$. Then there is $B$ such that $B^0 = C$ --- namely $C$
labelled everywhere by $0$. Since $M \real \forall a.\ \phi(a)$, we have
$\forall A \in V^\lambda.\ M\ reals \phi[a:=A]$. In particular, $M \reals
\phi[a:=B]$. By inductive hypothesis, $\phi^0[a:=B]$ holds, but
$\phi^0[a:=B] = \phi^0[a:=C]$. This ends the proof. 
\item $\exists a.\ \phi(a)$. Then there is $A$ such that $M \reals \phi(A)$,
so by IH, $\phi^0(A^0)$, so since $A^0$ is a set we get $\exists a.\
\phi^0(a)$. 
\end{itemize}
\end{proof}

\begin{lemma}
$IZF \proves (M \real \phi) \to M \downarrow$. 
\end{lemma}
\begin{proof}
Trivial. 
\end{proof}

\begin{lemma}
$M \downarrow v$ iff $IZF \proves M \downarrow v$.
\end{lemma}
\begin{proof}
$\Sigma_1$-completeness. 
\end{proof}

\begin{lemma}
$\gp M : \tau$ iff $IZF \proves (\gp M : \tau)$
\end{lemma}
\begin{proof}
$\Sigma_1$-completeness.
\end{proof}

\section{Sets and types and lambdas}

\begin{definition}
For any type $\tau$, we define a set $\SB{\tau}$ by structural induction on
$\tau$. Case $\tau$ of:
\begin{itemize}
\item $nat$ --- then $\SB{\tau} = \nat$ 
\item $\tau_1 \to \tau_2$ --- then $\SB{\tau} = \SB{\tau_1} \to \SB{\tau_2}$
\end{itemize}
\end{definition}

\begin{definition}[IZF]
For any map $\rho$ mapping variables to sets, we define
we define a set $\SB{M}_\rho$ for fully annotated term $M$ by structural induction on $M$. Case $M$ of:
\begin{itemize}
\item $x$ --- $\rho(x)$
\item $M\ N$ --- $\SB{N}_\rho\ \SB{O}_\rho$
\item $\lambda x : \tau.\ N$ --- $\{ (a, \SB{M}_{\rho[x:=a]})\ |\ a \in \SB{\tau} \}$.
\end{itemize}
\end{definition}

\begin{lemma}[IZF]
If $\gp M : \tau$ then for any $\rho \models \Gamma$, $\SB{M}_\rho \in
\SB{\tau}$. 
\end{lemma}
\begin{proof}
Induction on $\gp M : \tau$. 
\end{proof}

This lemma can modified to:

\begin{lemma}[HA]\label{lti}
If $\gp M : \tau$ then $IZF \proves \forall \rho \models \Gamma.\ \SB{M}_\rho \in
\SB{\tau}$. 
\end{lemma}
\begin{proof}
Trivial by the previous lemma and absoluteness of $\gp M : \tau$ --- we
simply inject the proof into the universe. 
\end{proof}

\input{dp}

\section{Going abstract}

We will be using many formal theories. It makes sense to point out the
formal properties important to us.

\begin{definition}
A \emph{formal theory} is any recursive set. 
\end{definition}

Some examples of formal theories we will use are the set of typing proofs $\{ \ov{\Gamma \proves M
: \tau} \}$ or the set of proofs in CZF/IZF $\{ \ov{\proves M } \}$.

\begin{definition}
A formal theory $A$ \emph{is functional} if the following conditions are
met:
\begin{itemize}
\item For any type $\tau$, there is a recursive subset $A_\tau$ of $A$.
\item There is a recursive operation $App : A_{\tau \to \sigma} \to A_\tau
\to A_\sigma$.
\end{itemize}
\end{definition}

The functionality of a theory is a much weaker requirement from even being a
category --- we don't require the functions to be composable, we don't
require the existence of identity functions. All we care about is the
possibility of applying a function to its argument.

\begin{example}
$\lst$ is functional. $A$ is a set of all typing proofs $\gp M : \tau$.
$A_\tau$ is a set of all proofs $\ov{\gp \proves M : \tau}$. The operation $App$
takes proof trees of $\ov{\proves M : \tau \to \sigma}$, $\ov{\proves N :
\tau}$ and returns a proof tree:
\[
\infer{M\ N : \sigma}
{
\infer{M : \tau \to \sigma}{} & \infer{N : \tau}{}
}
\]
\end{example}

\begin{example}
Any reasonable set theory $T$ with function spaces is functional. $A$ is a set of
all proofs. $A_\tau$ is a set of all proofs $T \proves t
\in \SB{\tau}$. The application operation take a proof $\ov{T \proves t \in
\SB{\tau} \to \SB{sigma}}$ and a proof that $\ov{T \proves s \in \SB{\tau}}$ and
returns the proof that $T \proves u \in \SB{\sigma}$, where $u$ is the unique 
element of $\SB{\sigma}$ such that $T \proves (s, u) \in t$. 
\end{example}

If $T$ formalizes types, then any $F \in A_{\tau \to \sigma}$ induces
in a natural way (using App) a function from $A_\tau$ to $A_\sigma$. Things
become interesting, when $T$ has an additional property:

\begin{definition}
A $T$ formalizing types is \emph{intuitionistic} if there is a pair of
recursive mappings $(f, g)$ such that:
\begin{itemize}
\item $f : \nat \to A_{nat}$.
\item $g : A_{nat} \to \nat$.
\item $g(f(n)) = n$. 
\end{itemize}
\end{definition}

\begin{example}
$\lst$ is intuitionistic. Indeed, $f$ is an injection of $n$ into a
proof:
\[
\infer{\proves n : nat}{}
\]
To define $g$, we know that $\lst$ strongly normalizes and has a subject
reduction property. Hence if $(\proves M : nat) \in A_\nat$, then $M \downarrow n$ for some
$n$. So take this $n$ as a value of $g$ on $M$. The check that $g \circ f = id$ is trivial. 
\end{example}

\begin{example}
CZF/IZF is intuitionistic. The function $f$ takes a natural number $n$ and produces
in one way or other the proof that $\ov{n} \in \nat$. The function $g$ uses
the procedure described in the previous section to extract a number from a
proof $IZF \proves t \in \nat$.

Even ZFC, understood as IZF + EM, is intuitionistic, when the sets $A_\tau$
are taken intact from IZF. 
\end{example}

When a theory is intuitionistic, any member $M$ of $A_{\tau_1 \to \tau_2 \to
{\ldots}  \to \tau_n \to \nat}$ defines a function of ``type'' $A_{\tau_1}
\to A_{\tau_2} \to {\ldots}  \to A_{\tau_n} \to nat$. Note that $nat$ in the
end --- we can actually extract a natural number. Moreover, by using
$f$, we can replace any $A_{\nat}$ by $nat$. Thus, in particular any $M :
\nat \to \nat$ actually induces a recursive function from $nat$ to $nat$. 

From now on, we consider only intuitionistic theories. We move on to a task
of comparing different formal theories. First we are going to compare
natural numbers in different theories in a natural way:

\begin{definition}
An injection $F$ of theory $S$ into a theory $T$ is a recursive family of
mappings $F_\tau : S_{\tau} \to T_{\tau}$.
\end{definition}

If there is an injection of $S$ into $T$ we can define (extensional) equality 
between member of respective types:

\begin{definition}
Let $F$ be an injection of $S$ into $T$. 
The extensional equiality relation $=_{F, S, T, \tau}$ is defined by structural induction on $\tau$.  Case $\tau$ of:
\begin{itemize}
\item $nat$ --- then $=_{F, S, T, nat} : S_{nat} \times T_{\nat}$ is defined as
follows: $M : nat =_{nat} N : nat$ iff $g(M) = g(N)$.
\item $\tau \to \sigma$ --- then $M : \tau \to \sigma
=_{F, S, T, \tau \to \sigma} N : \tau \to \sigma$ iff 
for all $O \in S_{tau}$, $App(M, O) =_\tau App(N, F(O))$. 
\end{itemize}
If the context is obvious, we will omit the subscripts from $=$ relation.
\end{definition}

\begin{definition}
A theory $S$ is a \emph{subtheory} of $T$ if there is an injection $F : S
\to T$ such that for all $\tau$, if $M \in A_\tau$ then $M =_{F, S, T, \tau} F(M)$.  
\end{definition}

\begin{lemma}
The relation of being a subtheory is reflexive and transitive. 
\end{lemma}

After these boring definitions, here's a chain of subtheories:
\[
\lst \subseteq \lambda^{\times, +} \subseteq MTT \subseteq CZF \subseteq IZF\\
\]

This shows that both intuitionistic set theories have hard computational
cores isomorphic to several standard lambda calculi/type theories.


==> setreal.tex <==
\section{IZF realizability as semantics for polymorphic type theory}

We will show that IZF realizability provides a natural semantics (and
consistency proof) for polymorphic type theory (CTT). 

We show first the result for CTT with simple types. The proof calculus is 
standard untyped lambda calculus with lazy evaluation. The proof system is as follows:

\[
\infer{\g, x : \tau \p x : \tau}{} \qquad
\infer{\gp M\ N : \sigma}{\gp M : \tau \to \sigma & \gp N : \tau} \qquad
\infer{\gp \lambda x. M : \tau \to \sigma}{\g, x : \tau \p M : \sigma} \qquad
\infer{\gp M : \tau}{\gp N : \tau & M \to N}
\]

We cannot apply Aczel interpretation here, since there is no reasonable way to
interpret in set theory full untyped lambda calculus, where typable terms
can contain $\Omega$ as subterms. However, the realizability interpretation
gives us alternative.

First, the arrow type should correspond to a function. We therefore define
for each type a set-theoretical sentence which will be realized. For more
clarity, we use set terms for this purpose. 

\begin{definition}
The set-term $\SB{\tau}$ for a type $\tau$ is defined by structural
induction on $\tau$. Case $\tau$ of:
\begin{itemize}
\item $a$ --- $\emptyset$.
\item $nat$ --- $\nat$.
\item $\tau \to \sigma$ --- $\{ f \in P(\SB{\tau} \times \SB{\sigma)}\ |\
\forall x \in \SB{\tau} \exists ! y \in \SB{\sigma}.\ (x, y) \in f \}$. 
\end{itemize}
\end{definition}

\begin{theorem}
Suppose $\gp M : \tau$. Let $\SB{\Gamma}$ denote $\SB{\tau_1} \times
\SB{\tau_2} \times {\ldots} \times \SB{\tau_n}$, where $\g = \{ x_1 :
\tau_1, {\ldots} , x_n : \tau_n \}$. Then there is a set-theoretical term $t$ and a realizer
$N$ such that $IZF \p N \reals t \in \SB{\g} \to \SB{\tau}$. 
\end{theorem}
\begin{proof}
Note that we do not really need set terms to state and prove this theorem. We
can think about them as metalevel abbreviation for the actual formula $
t \in \SB{\tau}$. For example, in this view, for $\tau = nat \to nat$, $t
\in \SB{\tau}$ is ``really'' ``$t$ is a set of pairs of natural numbers such
that for all $x \in \nat$ there is exactly one $y \in \nat$ such that $(x, y) \in
t$.''.

We proceed by induction on $\gp M : \tau$. Case $\gp M : \tau$ of:
\begin{itemize}
\item 
\[
\infer{\gp x_i : \tau_i}{}
\]
Then $t$ is the set $\{ ((x_1, {\ldots} , x_n), x_i) \in \SB{\g} \times
\SB{\tau_i}\}$. 

To exhibit a realizer $N$ we simply proceed with expanding the definitions.
The easiest way to do it, is to exhibit a normalizing proof in IZF of this
statement and get a realizer from the proof. We want to focus, though, on
one part of this realizer, namely $N \reals \forall x \in \SB{\g} \exists y \in \SB{\tau_i}.\ (x, y) \in t$.
If this is the case, then for all $A$, if $O \reals
A \in \SB{\g}$, then there is $B$ such that $N\ O \reals B \in \SB{\tau_i}
\land (A, B) \in t$. Now, if $O \reals A \in \SB{g}$, then
$O \reals \forall x \in A \exists \ov{y} \in \ov{tau}.\ x = \ov{y}$. 
So for all $C$, if $O \reals C \in A$, then there are $B_1, B_2, {\ldots} ,
B_n$ such that $N\ O \reals \ov{B} \in \SB{\ov{\tau}} \land C = <B_1, B_2, {\ldots} , B_n>$.
Then $\pi_{1i}(N\ O) \reals B_i \in \SB{\tau_i}$. Moreover, 




\end{itemize}

\end{proof}




==> subst.tex <==
\begin{lemma}\label{lamsl}
If $\Gamma, x : \tau \proves M : \sigma$ and  $\Gamma \proves N : \tau$, then $\Gamma \proves M[x:=N] : \sigma$.
\end{lemma}

\begin{proof}
By induction on $\gxp M : \sigma$. Case\footnote{Since
the type system is syntax-oriented, in proofs by induction on provability relation, we can do the proof by case
analysis of the form of the lambda term.} $M$ of:
\begin{itemize}
\item $a$. Impossible.
\item $x$. Since contexts are partial functions, we get that
necessarily $\sigma = \tau$, so since $x[x:=N] = N$ and $\Gamma \proves N :
\tau$, then also $\gp N : \sigma$.
\item $y \neq x$. Then $M[x:=N] = y$, a judgement $y:\sigma$ must be in $\Gamma$, so we get the claim as well.
\item $O\ P$. Then $\gxp O : \phi \to \sigma$ and $\gxp P : \phi$ for some
$\phi$. By IH, $\gp O[x:=N] : \phi \to \sigma$ and $\gp P[x:=N] : \phi$.
Therefore $\gp O[x:=N] P[x:=N] : \sigma$, so $\gp (O\ P)[x:=N] : \sigma$.
\item $\lambda y : \phi.\ O$, $y \neq x$, $y \notin FV(N)$. Then we have $\sigma = \phi \to
\psi$ for some $\psi$ and $\Gamma, x : \tau, y : \phi \proves O : \psi$. By
inductive hypothesis, $\Gamma, y : \phi \proves O[x:=N] : \psi$. Therefore, 
$\Gamma \proves \lambda y : \phi.\ O[x:=N] : \phi \to \psi$, so
also $\Gamma \proves M[x:=N] : \phi \to \psi$.
\item The cases for $<O, P>$, $fst(O), snd(O), inl(O), inr(O)$ work exactly like the case for
$O\ P$.
\item $case(O, y.P, y.Q)$, $y \neq x$, $y \notin FV(O\ P\ Q)$. Then we have
$\gxp O : \phi \lor \psi$, $\gx, y : \phi \proves P : \sigma$, $\gx, y :
\psi \proves Q : \sigma$. By IH, $\gp O[x:=N] : \phi \lor \psi$, $\Gamma, y
: \phi \proves P[x:=N] : \sigma$, $\Gamma, y : \psi \proves Q[x:=N] :
\sigma$. Therefore $\gp case(O[x:=N], y.P[x:=N], y.Q[x:=N]) : \sigma$, so
also\footnote{Note that we are using $\alpha$-conversion convention as here as in the
lambda-abstraction case extensively.} $\gp (case(O, y.P, y.Q)[x:=N] :
\sigma$.
\item $\lambda a. O$, $a \notin FV(N)$. Then $\sigma = \forall a.\ \phi$ for
some $\phi$. Also $\gxp M : \phi$. By IH, $\gp M[x:=N] : \phi$. So also $\gp
\forall a.\ M[x:=N] : \forall a.\ \phi$, so $\gp (\forall a.\ M)[x:=N] :
\forall a.\ \phi$.
\item $O\ t$. Then $\sigma = \phi[a:=t]$ for some $a$ and $\gxp O : \forall
a.\ \phi$. We may assume that $a \notin FV(M)$. By IH, $\gp O[x:=N] :
\forall a.\ \phi$. Therefore, $\gp O[x:=N] t : \sigma$ so also (since $t$ is
a logic term, it cannot have $x$ as a free variable) $\gp (O\ t)[x:=N] :
\forall a.\ \sigma$. 
\item $[t, O]$. Then $\sigma = \exists a.\ \phi$ and $\gxp O : \phi[a:=t]$
for some logic term $t$. By IH, $\gp O[x:=N] : \phi[a:=t]$, so $\gp [t,
O[x:=N] : \sigma$, so $\gp ([t, O])[x:=N] : \sigma$, which is what we want.
\item $let\ [a, z : \phi] := O\ in\ P$, $z \neq x$, $z \notin FV(N)$. Then $\gxp O : \exists a.\
\phi$, $\gx, z : \phi \proves P : \sigma$. By IH $\gp O[x:=N] : \exists a.\
\phi$. By IH again, $\Gamma, z : \phi \proves P[x:=N] : \sigma$. Therefore,
$\gp let\ [a, z : \phi] := O[x:=N]\ in\ P[x:=N] : \sigma$, so also 
$\gp (let\ [a, z : \phi] := O\ in\ P)[x:=N] : \sigma$.
\item The rest of the cases: $magic$, $aRep$, $aProp$for $a \in $ IZF
work exactly like the case for $O\ P$. 
\end{itemize}
\end{proof}

\begin{lemma}\label{logsl}
If $\gp O : \phi$ then  $\Gamma[a:=t] \proves O[a:=t] : \phi[a:=t]$.
\end{lemma}
\begin{proof}
By induction on $\gp O : \phi$. Case $O$ of:
\begin{itemize}
\item $a$ --- this case is impossible.
\item $x$. Then $(x, \phi) \in \Gamma$. Therefore $(x, \phi[a:=t]) \in
\Gamma[a:=t]$, so $\gp x : \phi[a:=t]$, which gives us the claim, since
$x[a:=t] = x$.
\item $M\ N$. Then $\gp M : \psi \to \phi$ and $\gp N : \psi$. By IH, $\gp
M[a:=t] : \psi[a:=t] \to \phi[a:=t]$ and $\gp N[a:=t] : \phi[a:=t]$, so
$\gp (M\ N)[a:=t] : \phi[a:=t]$ as well.
\item $\lambda x : \tau. P$, $x \notin FV(t)$ By inductive hypothesis, $\Gamma[a:=t], x :
\tau[a:=t] \proves P[a:=t] : \sigma[a:=t]$, where $\phi = \tau \to \sigma$. 
Therefore, $\Gamma[a:=t] \proves \lambda x : \tau[a:=t].\ P[a:=t] :
\tau[a:=t] \to \sigma[a:=t]$, so also $\gp (\lambda x : \tau.\ P)[a:=t] :
\phi[a:=t]$ which is what we want.
\item The cases for $<M, N>$, $fst\ M$, $inl\ M$ work just like the one for
application.
\item $case(M, x.N, x.P)$. Then $\gp M : \sigma \lor \tau$, $\Gamma, x :
\sigma \proves N : \phi$, $\Gamma, x : \tau \proves P : \phi$. By IH, $\gp
M[a:=t] : \sigma[a:=t] \lor \tau[a:=t]$, $\Gamma[a:=t], x : \sigma[a:=t]
\proves N[a:=t] : \phi[a:=t]$, $\Gamma[a:=t], x : \tau[a:=t] \proves P[a:=t]
: \phi[a:=t]$. Therefore $\gp case(M[a:=t], x.N[a:=t], x.P[a:=t]) :
\phi[a:=t]$ which, after pulling out the substitution from the case term is
what we want. 
\item $\lambda b.\ P$. We can assume that $b \notin FV(\Gamma) \cup \{a \}
\cup FV(t)$. Then $\Gamma \proves P : \sigma$, where $\phi =
\forall b.\ \sigma$. By inductive hypothesis, $\Gamma[a:=t] \proves M[a:=t]
: \sigma[a:=t]$. Since it is easy to see that $b \notin FV(\Gamma[a:=t])$, we
get $\Gamma[a:=t] \proves \forall z.\ M[a:=t] : \forall z.\ \sigma[a:=t]$ so also
$\Gamma[a:=t] \p (\forall z.\ M)[a:=t] : \phi[a:=t]$, which proves the claim. 
\item $M\ u$. Then $\gp M\ s : \phi[b:=u]$ and $\gp M : \forall b.\
\phi$ for some $b \notin FV(t) \cup \{a\}$. By IH, $\Gamma[a:=t] \proves M[a:=t] : \forall b.\ \phi[a:=t]$. Thus, 
$\Gamma[a:=t] \proves M[a:=t]\ u[a:=t] : \phi[a:=t][b:=u[a:=t]]$. By the
Formula Substitution Lemma we have $\phi[a:=t][b:=u[a:=t]] =
\phi[b:=u][a:=t]$. Pulling the substitution $[a:=t]$ out we now get the claim.
\item $[s, M]$. Then $\phi = \exists b.\ \psi$ and $\gp M : \psi[b:=s]$, $
\notin FV(t) \cup \{a\}$. By IH, $\Gamma[a:=t] \proves M[a:=t] : \psi[b:=s][a:=t]$. By Formula
Substitution Lemma we also have $\Gamma[a:=t] \proves M[a:=t] : \psi[a:=t][b:=s[a:=t]]$.
Therefore we have $\Gamma[a:=t] \proves [s[a:=t], M[a:=t]] : \exists b.\
\psi[a:=t]$ which in one step more gives us what we want. 
\item $let\ [b, x : \psi] := M\ in\ N$. We have $\gp M : \exists b.\
\psi[a:=t]$, $b \notin FV(t) \cup \{a\}$ and $\Gamma, x : \psi \proves N : \psi$. 
By IH we get $\Gamma[a:=t] \proves M[a:=t] : \exists b.\ \psi[a:=t]$,  and also
$\Gamma[a:=t], x : \psi[a:=t] \proves N[a:=t] : \psi[a:=t]$. Therefore,
$\Gamma[a:=t] \proves let\ [a, x : \psi[a:=t]] := M[a:=t]\ in\ N[a:=t] :
\psi[a:=t]$, which after pulling the subsitution out gives us the claim.
\item $magic(M)$. We have $\gp M : \bot$, so by IH $\gp M[a:=t] : \bot$, so
also $\gp magic(M[a:=t]) : \phi[a:=t]$. 
\item $aProp(s, \ov{u}, P)$. Then $\phi = \phi_A(s, \ov{u})$ and $\gp
P : s \in t_A(\ov{u})$. By inductive hypothesis, $\Gamma[a:=t] \proves
P[a:=t] : s[a:=t] \in (t_A(\ov{u}))[a:=t]$.
Therefore $\Gamma[a:=t] \proves aProp(s[a:=t], \ov{u}[a:=t], P[a:=t]) :
\phi_A(s[a:=t],
\ov{u}[a:=t])$. Pullling the substitution out of $\phi_A$ we get the claim. 
\item $aRep(t, \ov{u}, P)$. This proof is completely symmetric to the previous one.
\item $ind_{\psi(b, \ov{c})}(M, \ov{t})$. Then $\phi = \forall
b.\ \psi(b, \ov{t})$ and $\gp M : \forall c.\ (\forall b.\ b \in c \to
\psi(b, \ov{t})) \to \psi(c, \ov{t})$. By IH, $\gp M[a:=t] :
(\forall c.\ (\forall b.\ b \in c \to \psi(b, \ov{t})) \to
\psi(c, \ov{t}))[a:=t]$, so also, taking $c$ and $b$ not in $FV(t)
\cup \{ a \}$ and doing the same\footnote{That is $alpha$-renaming so that
there is no capture. And again, relying on the fact that all logic variables
of $\psi$ are displayed.}
inside of $\psi$, we get
$\gp M[a:=t] : \forall c.\ (\forall b.\ b \in c \to
\psi(b, \ov{t}[a:=t])) \to \psi(c, \ov{t}[a:=t])$. So also $\gp
ind_{\phi(b, \ov{c})}(M[a:=t], \ov{t}[a:=t]) : \forall b.\
\psi(b, \ov{t}[a:=t])$. Pulling the substitution out we get the claim.
\item $ind'_{\psi(b, \ov{c})}(M, \ov{t}, u)$. Similar to the
previous case.
\end{itemize}
\end{proof}


==> termsla.tex <==
\subsection{Terms}

The $\la$ terms are generated by the following grammar. 

\[
T ::= x\ |\ M\ N\ |\ \lambda x.\ M\ |\ inl(M)\ |\
inr(M)\ |\ fst(M)\ | \ snd(M)\ 
\]

\[
<M, N>\ |\ case(M, x.N, x.O)\ |\ magic(M)\ |\ 
\]

The terms generated by the part of the grammar above form the logical part
of $\li$. The terms used for IZF are listed below. 

\[
pairProp(M)\ |\ pairRep(M)\ 
sep_{\phi}Prop(M)\ |\ sep_{\phi}Rep(M)
\]

The free variables of a term are defined as usual, taking into account that:

\begin{itemize}
\item In $\lambda x : \tau.\ M$, $x$ is bound in $M$.
\item In $case(M, x.N, x.O)$, $x$ is bound in $N$ and $O$. 
\end{itemize}

The relation of $\alpha$-equivalence is defined taking this information into
account. 



==> tls.tex <==
\subsection{L axiom}

In this section we work in IZF0-L. Therefore, in particular we cannot
substitute equals for equals in the formulas we prove, so we need to be very
careful. The fact that equality is an equivalence relation follows without
L. We are using Kunen's notation and terminology. In particular, classes are
metalevel abbreviations for formulas defining them, for a class $M$,
$\phi^M$ means the formula $\phi$ with all quantifiers restricted to $M$ or,
more formally, if $M = \{ x\ |\ \psi_M(x) \}$, then $\phi^M$ results from
$\phi$ by changing each $\forall x.$ into $\forall x.\ \psi_M(x) \to$ and
each $\exists x.$ into $\exists x.\ \psi_M(x) \land$. Sometimes, instead of
saying that $\phi^M$ holds we will say $M \models \phi$, since intuitively
this is what it's supposed to mean. 


\begin{definition}
A set $C$ is L-stable if for all $a, b$, if $a \in C$ and $a = b$, then $b
\in C$. 
\end{definition}

\begin{definition}
A set $C$ is transitively L-stable (TLS) if it's L-stable and all its elements are
transitively L-stable. 
\end{definition}

Formally, this is not a valid definition of a predicate in first-order
logic. The valid definition of $TLS(C)$ uses the transitive closure of C,
denoted $TC(C)$ and defined in section 4 in \cite{ar}. It's important to
notice that Propositions 4.1. and 4.2. in \cite{ar} don't use (L) axiom. 
The definition is as follows:

\begin{definition}
TLS(C) holds iff $C$ is L-stable and for all $A \in TC(C)$, $A$ is L-stable. 
\end{definition}

The next pair of lemmas establish the equivalence of both definitions.

\begin{lemma}
If TLS(C) then C is L-stable and for any element B of C, TLS(B) holds.
\end{lemma}
\begin{proof}
That C is L-stable is obvious. Take any element $B$ of C. 
$B$ is also an element of $TC(C)$, so $B$ is L-stable. Now take any $A \in
TC(B)$. Since $TC(B) \subseteq TC(C)$, $A \in TC(C)$, so $A$ is L-stable as
well which ends the proof. 
\end{proof}

\begin{lemma}
If C is L-stable and for any element B of C TLS(B) holds, then TLS(C) holds. 
\end{lemma}
\begin{proof}
All that is to be shown is that if $A \in TC(C)$, then $A$ is L-stable.
By Proposition 4.2.2. in \cite{ar}, either $A \in C$ or there $A \in TC(x)$
for some $x \in C$. In the former case, we get the claim by $TLS(A)$. In the
latter, we have $TLS(x)$, so TLS(A) follows by the definition of the
predicate TLS.
\end{proof}

\begin{definition}
The class of all sets is denoted by V. 
The class of all transitively L-stable sets is denoted by T. The membership
and equality relations in T are the restrictions of the respective relations
in V. 
\end{definition}

\begin{lemma}
$T$ is transitive. 
\end{lemma}
\begin{proof}
Take any $A$ in $T$ and suppose $a \in A$. Then also $a \in T$, by the
definition of $T$. 
\end{proof}

\begin{lemma}\label{t1}
If $A=C$ and $A \in T$, then $C \in T$. 
\end{lemma}
\begin{proof}
Suppose $a \in C$ and $a = b$. Since $A=C$, $a \in A$. Since $A$ is
L-stable, $b \in A$, so also $b \in C$. Thus $C$ is L-stable. 

If $a \in C$, then $a \in A$. Since $A \in T$ and $T$ is transitive then $a
\in T$. Thus $C$ is transitively L-stable. 
\end{proof}

\begin{lemma}
$T$ is extensional, that is satisfies extensionality. 
\end{lemma}
\begin{proof}
Take any $A, B \in T$. If $A=B$, then for all $c$, $c \in A$ iff
$c \in B$. So in particular for all $c \in T$, $c \in A$ iff $c \in B$. 
On the other hand, suppose for all $c \in T$, $c \in A$ iff $c \in B$ and
take any $d$. If $d \in A$, then by transitivity of $T$, $d \in T$, so $d
\in B$. The other direction is similar.
\end{proof}

\begin{lemma}
$T$ satisfies Leibniz axiom, that is:
\[
\forall a, b, c.\ a \in c \to a = b \to b \in c
\]
\end{lemma}
\begin{proof}
Straightforward by the definition of $T$. 
\end{proof}

\begin{lemma}\label{l3}
$T$ satisfies full Leibniz axiom, that is for all $\phi(x, \ov{y})$:
\[
\forall \ov{q}, a, b.\ a = b \to \phi(a, \ov{q}) \to \phi(b, \ov{q})
\]
\end{lemma}
\begin{proof}
In the proof of Lemma \ref{ll} only (EXT) and (L) were needed which T
satisfies. 
\end{proof}

\begin{theorem}
$T \models IZF0$. 
\end{theorem}
\begin{proof}
We proceed axiom by axiom. We have already shown the claim for (EXT) and
(L). Since most of the axioms concern existence of certain sets, we do the
proofs in the similar way. First we show that the set in question exists,
then we show that it satisfies the respective axiom (in T). 
\begin{itemize}

\item (EMPTY) That $\emptyset$ is transitively L-stable is trivial. That it
is the empty set in T follows by absoluteness of open formulas. Just to make
sure, take any $a \in T$. If $a \in \emptyset$ then false and obviously if
false then $a \in \emptyset$. 
\item (PAIR) Take any $A, B \in T$. We show that\footnote{This is
IZF0, the set terms here are only metalevel abbreviations.} $\{ A, B \} \in
T$. 

Take any $a \in \{ A, B \}$ and suppose $a = b$. Then $a = A$ or $a = B$. So
either $b = A$ or $b = B$. In both cases $b \in \{ A, B \}$. Also, by Lemma \ref{t1}, $a
\in T$. 

That $\{ A, B \}$ satisfies the (PAIR) axiom in T follows by absoluteness of
equality. To be sure: take any $a, b, c \in T$. If $c \in \{ a, b \}$ then
$c = a$ or $c = b$. If $c = a$ or $c = b$ then $c \in \{ a, b \}$. 

\item For technical reasons, let's do (UNION) before (INF). Take any $A \in
T$, $a \in \bigcup A$, $a = b$. Since $a \in \bigcup A$, then $a \in d \in
A$ for some $d \in A$. By\footnote{This is the first time when we use
transitiveness of T in an essential way.} $A \in T$, $d \in T$, so also $a \in T$. By $d \in
T$, $b \in d$. That $\bigcup A$ satisfies its axiom in $T$ follows by
absoluteness of bounded formulas for transitive models of IZF0. 
\item (INF) We show that $\nat \in T$. Take any $a \in \nat$, $a = c$. We
show that $c \in \nat$ and $a \in T$ by $\in$-induction on $a$. Since $a \in \nat$, then $a = 0$ or there
is $b \in \nat$ such that $a = S(b)$. In the former case also $c = 0$, so $c
\in \nat$ and $a \in T$, since $0 \in T$, by Lemma \ref{t1}. In the latter,
$a = S(b)$ means really that $a = \bigcup \{ b, \{ b, b \} \}$. 
In particular, $b \in a$, since $b \in \bigcup \{ b, \{ b, b \} \}$, by $b \in
\{ b, b \}$ and $\{ b, b \} \in \bigcup \{b, \{ b, b \} \}$. By IH, $b \in
T$. We have $c \in \nat$, since there is $b$, $b \in \nat$ such that $c =
S(b)$, namely $b$. Since we have shown that $T$ is closed under pairing and union, $a \in
T$ as well.

Finally, we need to show that $\nat$ satisfies its respective axiom in T.
The claim follows by absoluteness of bounded formulas and notions used (0, S). 
\item (POWER) Take $A \in T$, we show that $P(A) \cap T \in T$. Take $a \in
P(A) \cap T$. Then obviously $a \in T$ and $a \subseteq A$. Suppose $a = b$, 
we need to show that $b \in P(A) \cap T$, that is first that $b \subseteq A$, that is any element 
of $b$ is an element of $A$. But any element of $b$ is an element of $a$ so also an element of $A$.
Second, that $b \in T$, but this follows by $a \in T$ and Lemma \ref{t1}. 

Now, for the defining axiom. Take any $a$. Suppose $a \in P(A) \cap T$. Then for all $x \in a$, $x
\in A$, so also for all $x \in T$, if $x \in a$, then $x \in A$. 

For the other direction, suppose that for all $x \in T$, if $x \in a$ then
$x \in A$. Obviously $a \in T$. To show that $a \in P(A)$, or that $a
\subseteq A$, take any $x \in a$. Then also $x \in T$, by $a \in T$. So $s
\in A$. This ends the proof. 
\item $(SEP_\phi)$. Take $\ov{B}, A \in T$, $a \in \{ x \in A\ |\ \phi^T(x,
\ov{B}) \}$. Then $a \in A$, so $a \in T$. Suppose $a = b$. We have $a \in A$
and $\phi^T(a, \ov{B})$. By $A \in T$, $b \in A$. By Lemma \ref{l3}, $\phi^T(b,
\ov{B})$. So also $b \in \{ x \in A\ |\ \phi^T(x, \ov{B}) \}$. And
obviously (precisely because we restrict the separation formula to $T$) this
set satisfies the respective separation axiom.
\item $(REPL_\phi)$. Take any $\ov{B}, A \in T$. Then the set $C = \{ z\ |
(\forall x \in A \exists! y \in T.\ \phi^T(x, y)) \land \exists x \in A.\
\phi^T(x, z) \}$ is in $T$. Indeed, let $a \in C$. Then
$T \models (\forall x \in A \exists! y.\ \phi(x, y)) \land \exists x \in A.\
\phi(x, a)$. Thus there is $d \in A$ such that $T \models \phi(d, a)$.
Also, there is $e \in T$ such that $\phi(d, e)$ and $e = a$. Thus $a \in T$. 

Now suppose $a = b$. We need to show that $b \in C$. To show that, we need
to show that $(\forall x \in A \exists! y \in T.\ \phi^T(x, y)) \land \exists x \in A.\
\phi^T(x, b) \}$. The first part of the conjuction is trivial. For the second
part, take $d$. We have $\phi^T(d, a)$. By Lemma \ref{l3}, we also have
$\phi^T(d, b)$ which is what we need.

Finally, $T \models \forall c. c \in C \iffl \forall x \in A \exists! y.\
\phi(x, y) \land \exists x \in A.\ \phi(x, c)$, since this is exactly the definition of $C$, taking into
account that we restrict in this definition $y$ and $\phi$ to $T$ (we don't
need to restrict $x$, since $T$ is transitive and already $A \in T$). This
ends the proof.
\item $(IND_\phi)$. Take $\ov{B} \in T$. Suppose that $\forall x \in T. 
(\forall y \in x.\
\phi^T(y, \ov{B})) \to \phi^T(x, \ov{B})$. We have to show that $\forall A.\ A \in T \to \phi^T(A, \ov{B})$.
We proceed by $\in$-induction on $A$. Take $A \in T$. By the assumption
instantiated with $A$, $(\forall y \in A.\ \phi^T(y, \ov{B})) \to \phi^T(A, \ov{B})$.
We have to show that $\phi^T(A, \ov{B})$. It suffices to show that $\forall
y \in A.\ \phi^T(y, \ov{B})$. But this follows immediately from the
inductive hypothesis (which is $\forall y \in A.\ y \in T \to \phi^T(y,
\ov{B})$) since $y \in A$ implies $y \in T$, by transitivity of $T$. 
\end{itemize}
\end{proof}

\begin{lemma}
Any set denoted by the expression generated by the following grammar:
\[
A ::= \emptyset\ |\ \{ A, B \}\ |\ \nat\ | \bigcup A
\]
is in T and is absolute for T. We call any such set $T$-stable. 
\end{lemma}
\begin{proof}
We have shown essentially in the previous lemma that any $T$-stable set is
in $T$ and satisfies its respective axiom, which in IZF0-L can be strengthened to be a
defining one. 
\end{proof}

\begin{theorem}[(ZFC)]\label{zfc}
Let $\phi$ be an absolute formula for $T$, containing T-stable constants. Then $IZF0 \proves \phi$ iff $IZF0-L \proves \phi$. 
\end{theorem}
\begin{proof}
One direction is trivial. For other, suppose $IZF0 \proves \phi$. Take any
model $M$ of IZF0-L. Let $N$ be $T$ inside of $M$. By $N \models IZF0$ and
soundness $N \models \phi$. This means that $M \models \phi^N$. By
absoluteness of $\phi^N$, $M \models \phi$. By completeness, since $M$ was
an arbitrary model of IZF0-L, $IZF0-L \proves \phi$. 
\end{proof}

\begin{corollary}
$IZF0$ is arithmetically conservative over $IZF0-L$. In other words, if
$IZF0 \proves \phi$, where $\phi$ is an arithmetical sentence, then $IZF0-L
\proves \phi$ as well. 
\end{corollary}
\begin{proof}
By Theorem \ref{zfc}, $\nat$ being $T$-stable and absoluteness of bounded
formulas. 
\end{proof}


==> typeslz.tex <==
\subsection{Typing system}

This section contains the typing system for $\li$. Types are IZF formulas.
In $\li$, contexts are sequences of $x_1 : \tau_1, {\ldots} , x_n : \tau_n$,
where no variable appears twice. The \emph{range} of a context $\g$ is the
corresponding IZF context which contains only formulas and is denoted by $rg(\Gamma)$.
The \emph{domain} of a context $\g$ contains of lambda variables of $\g$ and
is denoted by $dom(\g)$. The free variables of a
context $\g$, denoted by $FV(\g)$ are defined as $FV(rg(\Gamma))$. 

Apart from standard judgements, the typing system also contains judgements
of the form $\gp t : Set$. In a judgement like this, $Set$ is
\emph{not} a type, rather a kind. These judgements are included only to make
the presentation (especially the normalization proof) more smooth.

\[
\infer{\g, x : \tau \p x : \tau}{} \qquad \infer{\gp M\ N : \tau}{\gp M : \sigma \to
\tau & \gp N : \sigma} \qquad \infer{\gp \lambda x : \tau. M : \tau \to
\sigma}{\g, x : \tau \p M : \sigma}
\]

\[
\infer{\gp <M, N> : (\tau, \sigma)}{\gp M : \tau & \gp N : \sigma} \qquad
\infer{\gp fst(M) : \tau}{\gp M : (\tau, \sigma)} \qquad \infer{\gp snd(M) :
\tau}{\gp M : (\tau, \sigma)}
\]

\[
\infer{\gp inl(M) : \tau \lor \sigma}{\gp M : \tau} \qquad \infer{\gp inr(M) : \tau \lor
\sigma}{\gp M : \tau} \qquad \infer{\gp case(M, x.N, x.O) : \tau}{\gp M :
\sigma \lor \rho & \g, x : \sigma \proves N : \tau & \g, x : \rho \proves O : \tau}
\]

\[
\infer[a \notin FV(\Gamma)]{\gp \lambda a.\ M : \forall a.\
\sigma}{\gp M : \sigma} \qquad \infer{\gp M\ t :
\phi[a:=t]}{\gp M : \forall a.\ \phi & \gp t : Set}
\]

\[
\infer{\gp [t, M] : \exists a.\ \phi}{\gp M : \phi[a:=t] & \gp t : Set}
\qquad \infer[a \notin FV(\Gamma, \psi)]{\gp let\ [a, x : \phi] := M\ in\
N : \psi}{\gp M : \exists a.\ \phi & \Gamma,  x : \phi \proves N : \psi}
\]

\[
\infer{\gp magic(M) : \phi}{\gp M : \bot} \qquad \infer{\gp t : Set}{} 
\]

\[
\infer{\gp pairRep(t, u_1, u_2, M) : t \in \{ u_1, u_2 \}}{\gp M : t = u_1
\lor t = u_2) & \gp t : Set & \gp : u_1, u_2 : Set}
\qquad \infer{\gp pairProp(t, u_1, u_2, M) : t = u_1 \lor t = u_2}{ \gp M : t
\in \{ u_1, u_2 \} & \gp t : Set & \gp : u_1, u_2 : Set}
\]

\[
\infer{\gp sep_{\phi(z, \ov{y})}Rep(t, u, \ov{u}, M) : t \in sep_{\phi(z, \ov{y}}(u, \ov{u})}
{\gp M : t \in u \land \phi(t, \ov{u}) & \gp t, u : Set & \gp \ov{u} : Set}
\qquad 
\infer{\gp sep_{\phi(z, \ov{y})}Prop(t, u, \ov{u}, M) : t \in u \land \phi(t, \ov{u})}
{\gp M : t \in sep_{\phi(z, \ov{y}}(u, \ov{u}) & \gp t, u : Set & \gp
\ov{u} : Set}
\]


